Causal Relational Learning

Causal inference is at the heart of empirical research in natural and social sciences and is critical for scientific discovery and informed decision making. The gold standard in causal inference is performing randomized controlled trials; unfortunately these are not always feasible due to ethical, legal, or cost constraints. As an alternative, methodologies for causal inference from observational data have been developed in statistical studies and social sciences. However, existing methods critically rely on restrictive assumptions such as the study population consisting of homogeneous elements that can be represented in a single flat table, where each row is referred to as a unit. In contrast, in many real-world settings, the study domain naturally consists of heterogeneous elements with complex relational structure, where the data is naturally represented in multiple related tables. In this paper, we present a formal framework for causal inference from such relational data. We propose a declarative language called CaRL for capturing causal background knowledge and assumptions and specifying causal queries using simple Datalog-like rules.CaRL provides a foundation for inferring causality and reasoning about the effect of complex interventions in relational domains. We present an extensive experimental evaluation on real relational data to illustrate the applicability of CaRL in social sciences and healthcare.

==> Background.tex <==
\vspace{-0.3cm}
\section{Background on Causal Analysis}\label{sec:background}
% lg1 - this is repetitive, it needs a very strong pass of removing
% redundant bits
%
\red{{\LARGE $1.5$ pages}}\
In this section we \revm{review fundamental concepts in causal analysis.} \revm{We use capital letters $X,Y,$ etc., to denote \revm{random} variables, and use with lower case $x, y,$ etc. to denote their values.  We use boldface $\mb X$, $\mb x$ (etc.) to denote tuples of random variables and constants respectively; and \revm{$Dom(X)$ denotes the domain of variable $X$. 
%We use $X \indep Y$ to denote that $X, Y$ are two independent variables, and $X \indep Y|Z$ to denote their conditional independence given $Z$.
}
%\revm{We denote \revm{random} variables with capital letters $X,Y,$ etc., and their values (constants) with lower case $x, y,$ etc.  We use boldface $\mb X$, $\mb x$ (etc.) to denote tuples of random variables and constants respectively; \revm{$Dom(X)$ denotes the domain of variable $X$. 
%We use $X \indep Y$ to denote that $X, Y$ are two independent variables, and $X \indep Y|Z$ to denote their conditional independence given $Z$.
}


% lg1 - I don't see why we have to have all theses multiple names for something, why do we have to call it
% x or y.   Let's just pick one.   Since the issue is terminology overload, only include terminology that is needed
%
% Our framework for going beyond the restrictive assumption of homogeneous units in traditional causal inference is grounded in Pearl’s causality which we review in this section.
% \paragraph*{\bf Treatments, potential outcome,  intervention, and average treatment effect (ATE)}
\paragraph*{\bf Potential outcome and treatment effect}
\revm{ 
%The notion of causality both by Pearl \cite{pearl2009causality} and Rubin  \cite{rubin2005causal} is built on the
The notion of causality %both by Pearl \cite{pearl2009causality} and Rubin  \cite{rubin2005causal} 
is built on the idea of \emph{units}, or physical objects of interest (e.g., patients, publications, etc.).
Units can be exposed to \emph{treatments}, denoted $T$.   Treatments may then effect 
idea of \emph{intervention} of a \emph{treatment} variable $T$ on
a \emph{response} or an \emph{outcome} variable $Y$. 
There are a set of \emph{units} or physical objects of interests (e.g., people or publications) at a particular time point.  Each unit can be exposed to the treatment $T$ (called \emph{active treatment}, $T = 1$, and the unit is called a \emph{treated unit}) or not (called \emph{control treatment}, $T = 0$, and the unit is a \emph{control unit}). Rubin's model defines the \emph{potential outcomes} as the value of the outcome variable $Y$ for each unit after the active treatment or control treatment has been applied, denoted by $Y(1)$ and $Y(0)$ under the active and control treatment respectively (i.e., $Y = TY(1) + (1-T)Y(0)$). Pearl's model defines an equivalent form of intervention or counterfactual using the \emph{do-operator} (discussed in detail below in terms of a causal graph) expressed as $Y | do(T = 1)$ and $Y | do(T = 0)$ for active and control treatment respectively. A standard goal in causal analysis is to compute the \emph{Average Treatment Effect (ATE)} expressed as follows:
{\footnotesize
\begin{eqnarray}
\ate(Y, T) =  \Ex[Y(1) - Y(0)] %\nonumber\\
 =  \Ex[Y|do( T= 1)]-\Ex[ Y|do( T= 0)] 
\label{eq:ate}
\end{eqnarray}
}
}
\revm{\textbf{Observational causal analysis.~} For any unit under consideration, only one of the potential outcomes $Y(1)$ or $Y(0)$ can be observed -- only $Y(1)$ can be observed for a treated unit whereas only $Y(0)$ can be observed for a control unit. This makes causal analysis or the computation of ATE (\ref{eq:ate}) a \emph{missing data problem}. For randomized controlled trials (which are used, e.g., to understand the effectiveness of a new drug) this problem is easily solved as treatment $T$ is assigned at random to the units, i.e., $Y(1), Y(0) \indep T$ where the symbol $\indep$ denotes independence\footnote{\revm{The potential outcomes $Y(1), Y(0)$ are independent of the `assignment' of treatment $T$, not the treatment itself.}}, and therefore under assumptions called \emph{SUTVA}\footnote{\revm{\emph{SUTVA} or \emph{Stable Unit Treatment Value Assumption} by Rubin \cite{rubin2005causal} assumes that (1) there is no \emph{interference}
between units, \ie, $Y(1)$  or $Y(0)$ of any unit is not affected by what treatment action the other units received, and (2) there are no hidden versions of treatments,  i.e.,  for a treatment (control)  unit  the response will be $Y(1)$ ($Y(0)$) irrespective of how it received the treatment.} }  \cite{rubin2005causal} (\ref{eq:ate}) reduces to 
{\small
\begin{equation}
    \ate(Y, T) = \Ex[Y(1) - Y(0) | T] = \Ex[Y| T = 1] - \Ex[Y | T = 0] 
\end{equation}
}
which can be easily estimated from the observed data. However, due to ethical, time, or cost constraints, randomized controlled trials are not feasible for many causal questions of interests like whether smoking causes cancer. Although for many such questions historical \emph{observational} or \emph{collected} data is available, since the treatment $T$ may not be assigned at random, the above expression for \ate\ no longer holds (e.g., males of a certain age range are more likely to be smoker than others). Fortunately, it has been observed by both Pearl's and Rubin's causal models that sound causal analysis is still possible on observational data under some assumptions by recording possible variables   that can affect assignment of treatments to units (called \emph{confounding covariates}). If such variables $\mb X$ are observed, then under the assumption that $Y(1), Y(0) \indep \mb X | T$ (called \emph{strong ignorability} \cite{Rubin1983b}), (\ref{eq:ate}) becomes
{\footnotesize
\begin{eqnarray}
\ate(Y, T)  =  \Ex_{\mb X}[\Ex[Y(1) - Y(0) | T, \mb X] 
 =  \Ex[Y| T = 1, \mb X] - \Ex[Y | T = 0, \mb X]] \label{eq:string-ignorability}
\end{eqnarray}
}
which can again be estimated from the observed data. 
}
% \paragraph*{\bf Probabilistic causal model, causal DAGs, and do - operator}
\paragraph*{\bf Probabilistic causal model and do - operator}
\revm{Next we discuss probabilistic causal model by Pearl \cite{pearl2009causality} that allows fine-grained causal relationships among possible confounding covariates $\mb X$ themselves based on background knowledge of the users giving guidance on what to condition on in observational causal analysis. } A probabilistic causal model \cite{pearl2009causality} is a tuple
$\cm = \langle \mb U, \mb V , \mb F, \pr_{\mb U} \rangle$, where \revm{
$\mb U$ is a set of \emph{exogenous} variables that cannot be observed,  
$\mb V$ is a set of \emph{observable or endogenous} variables, $\mb F$ is a set of \emph{non-parametric  structural equations}, and $\pr_{\mb U}$
is a joint probability distribution on the exogenous variables
$\mb U$. The set $\mb F = (F_X)_{X \in \mb V}$ 
%is a set of \emph{non-parametric  structural equations}
comprises structural  equations of the form 
$F_X : Dom(\Pa_{\mb V}(X)) \times Dom(\Pa_{\mb U}(X)) \rightarrow
Dom(X)$, where  $\Pa_{\mb U}(X) \subseteq \mb{U}$ and
$\Pa_{\mb V}(X) \subseteq \mb V-\set{X}$ are called the \textit{exogenous
parents} and \textit{endogenous parents} of $X$ respectively.}
Intuitively, the exogenous variables $\mb U$ are not known,
but we know their probability distribution; the endogenous
variables are completely determined by their parents (exogenous and/or
endogenous). 
\cutr{
\sout{In this paper, given users' background knowledge and assumptions about causal models, we use observational data to validate assumptions and quantify causal effects. Background knowledge is {\em fundamentally} required for causal inference \cutr{\cite{pearl2009causal, rubin2005causal}}
}
}
A probabilistic causal model is
associated with a {\em causal graph}, $\cg$, whose nodes are the
endogenous variables $\mb V$, and whose edges are all pairs $(Z,X)$
such that $Z \in \Pa_{\mb V}(X)$. \cutr{We write $Z \rightarrow X$ for an
edge;} 
It is usually assumed that $\cg$ is acyclic which, in that case, is
called a Causal DAG  \revm{(directed acyclic graph)}.  In other words, the causal DAG hides
exogenous variables (since we cannot observe them anyway) and instead
captures their effect by defining a probability distribution
\revm{$\pr_{\mb U}$} on the endogenous variables.  This is possible under the
{\em causal sufficiency} assumption.\footnote{The assumption requires
  that, for any two variables $X, Y \in \mb{V}$, their exogenous
  parents are disjoint and independent
  $\Pa_{\mb U}(X) \indep \Pa_{\mb U}(Y)$.  When this assumption fails,
  one adds more endogenous variables to the model to expose their
  dependencies.}
\revm{We will only refer to endogenous variables in the rest of the paper
and drop the subscript $\mb{V}$ from $\Pa_{\mb{V}}$. 
%and $\pr_{\mb{V}}$.}  
Similarly,  we will  drop the subscript $\mb U$ from the probability distribution $\pr_{\mb U}$ when it is clear from the context.}
Then the formula for $\pr(\mb V)$ is the same as that
for a Bayesian network:

%\revm{(where $\prod$ denotes the joint distribution)}
% 

%
\vspace{-0.2cm}
{\footnotesize
\begin{align}
\pr(\mb V) = & \prod_{X \in \mb V} \pr(X | \Pa(X))  \label{eq:bayesian}
\end{align}
}
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.2]{Figures/causal-dag-simple}
    \vspace{-2mm}
    \caption{A standard %and simple 
    causal DAG for Example~\ref{eg:instance}. 
    %\red{SR: Make the height smaller}
    }
    \vspace{-5mm}
    %\dan{done}\babak{thanks Dan the comments was for Moe!}
    \label{fig:simple-causal-dag}
\end{figure}

\par
Figure~\ref{fig:simple-causal-dag} shows a simple
example of a causal graph \revm{based  on Example~\ref{ex:univdomain:causalmodel}: the Score of a paper is affected by its
Quality and by the Prestige of the author (assuming the reviews are
single blind), whereas both Quality and Prestige are affected by the author's
Qualification. Here $\mb V$ = \{\texttt{Qualification}, \texttt{Quality}, \texttt{Prestige}, \texttt{Score}\} are endogenous variables, $\mb U$ endogenous variables are unknown (e.g., mood of a reviewer while reviewing the paper, the expected number of papers to be accepted, scores of other papers the reviewer reviewed, etc.) leading to a probability distribution on $\mb V$. The  dependencies can be represented by three structural  equations:
%form can be represented as:
{\scriptsize
\begin{equation}\label{eq:se_background}
\text{Quality} \sem   \text{Qualification};~
\text{Prestige} \sem  \text{Qualification};~
\text{Score} \sem  \text{Quality}, \text{Prestige}
\end{equation}
}
\cutr{
{\footnotesize
\begin{eqnarray} 
\text{Quality} &\sem &  \text{Qualification}\nonumber\\
\text{Prestige} &\sem & \text{Qualification}\nonumber\\
\text{Score} &\sem & \text{Quality}, \text{Prestige}\label{eq:se_background}
\end{eqnarray}
}
}
}




\cut{In this paper we will assume that the causal DAG is
known,\footnote{There exists an extensive literature on learning the
  causal DAG from data.} and one uses some observational data in
order to learn the conditional probability distribution
(\ref{eq:bayesian}).}  




%\paragraph*{\bf Causal DAG} 
\cutr{The probabilistic causal model is
associated with a {\em causal graph}, $\cg$, whose nodes are the
endogenous variables $\mb V$, and whose edges are all pairs $(Z,X)$
such that $Z \in \Pa_{\mb V}(X)$.
}

%\vspace{-0.35cm}

%
% Thus justifies omitting the exogenous variables from the causal DAG,
% and capturing their effect through the probability distribution in
% (\ref{eq:bayesian}).  


% A {\em path} in $\cg$ means an undirected path, i.e. we may traverse edges either forwards or backwards; a {\em directed path} is one where we traverse edges only forwards. 

%{\em Acyclicity}: Although our language is rich enough to express complex cyclic causal relationship that involve with feed-back and contagion, in this paper we assume $\gcg(\rcm^{\skl})$ is acyclic. %A common inference question in a causal DAG is how to determine whether a
%CI $(\mb X \indep \mb Y | \mb Z)$ holds.  A sufficient criterion is
%given by the notion of {\em d-separation},  a syntactic condition
%$(\mb X \indep \mb Y |_G \mb Z)$ that can be checked directly on he
%graph (see \cite{pearl2009causal} for details). 
%\vspace{-0.2cm}

\cutr{
\paragraph*{\bf $d$-Separation and  Markov compatibility} 
\sout{A common inference question in a causal DAG is how to determine whether a
CI $(\mb X \indep \mb Y | \mb Z)$ holds.  A sufficient criterion is
given by the notion of d-separation,  a syntactic condition
$(\mb X \indep \mb Y |_d \mb Z)$ that can be checked directly on the
graph.  $\pr$ and $\cg$ are
called {\em Markov compatible} if $(\mb X \indep \mb Y |_d \mb Z)$
implies $(\mb X \indep_\pr \mb Y | \mb Z)$; if the converse
implication holds, then we say that $\pr$ is {\em faithful} to $\cg$.
The following is known: 
}
}
\cutr{
\begin{proposition} \label{prop:d:separation}
\sout{If $\cg$ is a causal DAG and
  $\Pr$ is given by Eq.(\ref{eq:bayesian}), then they are Markov
  compatible.
  }
\end{proposition}
}

\vspace{-0.2cm}
%\paragraph*{\bf Interventions and the \texttt{do} operator}
In this causal model, an  intervention represents actively setting an
endogenous variable to some fixed value and observing the effect denoted by the $do$-operator introduced by 
Pearl~\cite{pearl2009causal}.
%introduced for this purpose the $do$-operator.  
Formally, an intervention \revm{$\Do(\mb W = \mb w)$} consists of setting
variables \revm{$\mb W \subseteq \mb V$} to some values \revm{$\mb W= \mb w$}, and it defines the
probability distribution \revm{$\pr(\mb V | \Do(\mb W = \mb w))$} given by
(\ref{eq:bayesian}), where we remove all factors $\pr(X | \Pa(X))$,
where $X \in \mb W$.  In other words, we modify the causal DAG by
``removing all edges entering the variables $\mb W$ on which we intervene; this fundamentally differs from conditioning,
\revm{$\pr(\mb V | \mb W = \mb w)$}.  Pearl has an extensive discussion of
the rationale for the $do$-operator and describes several equivalent
formulas for estimating the effect of \revm{$\Do(\mb W = \mb w)$} from \revm{an} observed distribution \cite{pearl2009causality}.

%\babak{Sudeepa: we need D-separation for the theorem in section 5.1 (not just for the proof). Also I think the background must be significantly shortened}

% In a causal DAG $G$, this intervention is denoted by
% $\Do(\mb X=\mb x)$ which replaces the conditional probability
% distributions $\pr(X | \Pa(X))$ for $X \in \mb X$ with
% constants. Then, it is implied from the factorization
% (\ref{eq:bayesian}) that the counterfactual distribution
% $\pr(\mb V |do(\mb X=\mb x))$ can be always {\em identified} as the
% following function of the observed distribution $\pr(\mb V)$
% (observational data) \cite{pearl2009causality}:
% 
% 
% is a surgical operation that changes the state of a
% set of variables $\mb X$ in the real world to some value
% $\mb X= \mb x$. In a causal DAG $G$, this intervention is denoted by
% $\Do(\mb X=\mb x)$ which replaces the conditional probability
% distributions $\pr(X | \Pa(X))$ for $X \in \mb X$ with
% constants. Then, it is implied from the factorization
% (\ref{eq:bayesian}) that the counterfactual distribution
% $\pr(\mb V |do(\mb X=\mb x))$ can be always {\em identified} as the
% following function of the observed distribution $\pr(\mb V)$
% (observational data) \cite{pearl2009causality}:
% %i
% \begin{align}
% \pr(\mb V |do(\mb X=\mb x))& =\frac{\pr(\mb V)}{ \prod_{X \in \mb X} \Do(\mb X=\mb x)} 
% \label{eq:indet}
% \end{align}
% 
%
\cutr{
\vspace{-0.2cm}
\paragraph*{\bf Average Treatment Effect (ATE)}
\sout{Rubin's Potential Outcome Framework~\cite{rubin1970thesis}
compares the effect of a binary treatment variable $T$ on some response
variable $Y$. This effect is often measured by the following quantity known
as the {\em average treatment effect (ATE)}, which is
expressed as follows in our notation:}
%
\begin{align}
\ate(Y, T)& = \Ex[Y|do( T= 1)]-\Ex[ Y|do( T= 0)] 
\label{eq:ate}
\end{align}
%
\sout{Much of the literature on Rubin's Potential Outcome Framework in statistics addresses efficient estimation of $\ate$ from observational data.}
}

%
%
%Much of the literature on the Neyman-Rubin causal model in statistics is concerned with finding sufficient conditions under which $\ate$ can be estimated efficiently from the existing, observational data.
%
%
% Now, the counterfactual distributions $\pr(Y|do( T= t))$ for $t=\{0,1\}$, identified from (\ref{eq:indet}) by marginalisation. Note that in practice, the RHS of (\ref{eq:indet}) needs to be carefully transformed to a probabilistic formula in terms of {\em low-dimensional (conditional)  probability distributions} that can be estimated from limited data using the existing techniques in ML and Statistics (see section~\ref{sec:cov-detec}).
\paragraph*{\bf Other related work and contributions of this paper over previous work}
\revm{A fundamental limitation of traditional
causal frameworks is that they assume the units of analysis are \emph{homogeneous} and satisfy SUTVA \cite{rubin2005causal}, i.e., there can be only one type of units (like tuples in a single relational table) and the units do not interfere with one other. 
Therefore, these models can not be used for causal inference in relational domains
that involve heterogeneous units with complex causal dependencies and interference.
%that involve with interference. 
In Example~\ref{ex:univdomain:causalmodel}, we have heterogeneous entities such as authors, submissions, conference that are relationally connected. To answer causal questions such as what is the effect of author's prestige on their submission score it is even not clear whether the authors or submissions should be regarded as units of analysis. Moreover, selecting authors as the units of analysis would lead to violation of  SUTVA. This is because the review scores associated to one author is not only affected by his or her own prestige but also influenced by  his or her collaborators' prestige. Therefore, situations like multiple authors for the same paper, multiple submissions by the same authors, or multiple reviews received by the same paper cannot be represented in traditional causal inference framework.
Some previous works studied causal inference in the presence of interference \cite{ogburn2017causal,graham2010measuring,halloran2012causal,halloran1995causal,tchetgen2012causal,vanderweele2011bounding,aronow2017,shalizi2011homophily,ogburn2014causal,ogburn2018causal}. These works address applications such as the study of infectious diseases \cite{vanderweele2011bounding, halloran1995causal} or behavior and interactions in social networks \cite{shalizi2011homophily,ogburn2018causal, sobel2006randomized,graham2010measuring, vanderweele2011bounding, maier2013reasoning,hong2006evaluating}. But in these studies the units are still homogeneous (e.g., people connected by a social network), and they are unable to capture different \emph{entities} of interests like papers, authors, reviews and their complex many-to-many relationships that we focus on \sys.
\cutr{The novel contribution of this paper is to bridge the gap between  relational data model and observational causal studies by proposing a simple declarative framework  that enables sound but easier causal analysis for multi-relational  data frequently encountered in practice.
}.
}
There has been prior work on learning causality from relational data \cite{maier2013sound,DBLP:conf/uai/2019,lee2016learning,maier2010learning}; {it focuses on discovering the structure of probabilistic graphical models for this data. These models were originally proposed for Statistical Relational Learning, which aims to model a joint probability distribution over relational data amenable for probabilistic reasoning rather than causal inference ~\cite{Getoor:2007:ISR:1296231}. \revd{This line of work differs from our work in that our objective is develop a declarative framework to answer complex causal queries about the effect of interventions, given the existing background knowledge}. 
\cutr{\sout{\sys\ extends existing literature by: (1) relaxing the assumption of homogeneous units with one type of relationship in interference literature to heterogeneous units with different types of relationships, (2) using a declarative language to represent complex causal dependencies such as interference and contagion, that cannot be succinctly expressed using graphical models for relational data and (3) articulating the assumptions and conditions needed to infer causality from relational data.}
}
Note that {\em causality} has been used in various contexts \cite{meliou2014causality}, namely,  to understand responsibility in query answering  \cite{MeliouGMS2011, SalimiTaPP16}, in database repair \cite{meliou2011tracing, DBLP:conf/icdt/SalimiB15}, and to motivate explanations \cite{RoyS14}. It has also inspired different applications such as  hypothetical reasoning \cite{balmin2000hypothetical,lakshmanan2008if, deutch2013caravan, meliou2012tiresias}. These differ from our work in that they identify parts of the input that are correlated with output of a transformation, which is useful but %insufficient for decision making.
\revm{does not reflect the true causality needed for decision makings.}

%\red{SR: To revise the paragraph above and polish this section, see if  Dom can be removed from  structural equations.}


 

%


==> Related.tex <==

%has been extensively studies in the literature . Here the aim is to unifying logic and statistics to learn a joint probability distribution over relational data.


%Traditional machine learning algorithms fit a function from a feature vector to a response prediction. statistical relational learning aims at unifying logic and statistics to enable probabilistic reasoning in relational data. It has been successfully applied to several applications such as entity resolution, knowledge graph completion .. 





%\par
%\textbf{\bf Extenuation to Cyclic RelCM.} 
%The acyclicity assumptions can be violated in relational domain in which units that are relationally connected shows contagious behavior. Much literature addresses cyclic causal models, \eg, \cite{spirtes1995directed,richardson1996discovery,bongers2018theoretical}. In \sys\ we use an alternative formulation of feed-back loops using equilibrium of discrete Markov chains. Even though our formulation is fully equipped to handle the feedback loops, due to lack of space we restrict our attention to acyclic RelCM. We defer the extension to cyclic RelCMs to the extended version of this paper. 

%\par



%As discussed in example~\ref{ex:univer_schema2}, the structural equation defining the endogeniety of a student's attendance in a course has a feedback nature by the definition i.e. the attendance of one student is dependent on their friends' attendance and the friend's attendance by same reasoning is dependent on their reasoning.

%\red{Discuss TOP K PeerS from 4.2}


\section{Conclusions And future work}
%
%\red{SR: UPDATE} 
\revm{We introduced \emph{\sys\ (Causal Relational Language)}, a declarative language for representing casual background knowledge  in relational domains 
%and to ask  %Using \sys\ 
%complex causal models can be specified 
using %just a few  
simple Datalog-like rules, and for asking various complex causal queries on relational data.}
%about the isolated and relational effects of interventions can be specified in a declarative language.  
\sys\ extends existing literature in causal inference by relaxing the assumption of homogeneous units with one type of relationship in interference literature to heterogeneous units with different types of relationships, (2) using a declarative language to represent complex causal dependencies such as interference and contagion, that cannot be succinctly expressed using graphical models for relational data and (3) articulating the assumptions and conditions needed to infer causality from relational data.\cut{Our experimental results show that ignoring the relationality of data and using traditional methods for causal inference can indeed lead to false discoveries that can be avoided using \sys.}
%We gave semantics to the relational causal queries by proposing a new, non-trivial extension of Pearl's
%$\Do$-operator to relational causal models.  We proposed an algorithm for evaluating causal queries from the given data, by creating on-the-fly a table of units (specific to the query) and
%finding a sufficient set of {\em covariates} that should be adjusted
%for to remove confounding effects. 

In future work, we aim to extend \sys\ to deal with complex cyclic causal dependencies using stationary distribution of stochastic  processes.  We plan to study  stochastic interventions and complex interventions on relational skeletons, which are assumed to be fixed in this paper.  We also plan to study more complex methods for embedding such as using recurrent neural networks and graph convolutional networks. 

==> Sys.tex <==
\subsection*{Challenges}
\label{eq:challanges}
\babak{Placeholder. Ignore for now}

In this section, we discuss the methodological and technical challenges in applying the existing approach for causal inference to relational data. 


The most prominent approach for causal inference in statistics in the POF, which 
relies on the concept of {\em unit} defined as a physical object or entity, for example, a patient, at a particular place and point of time~\cite{rubin2008objective}. Other central concepts such as treatment, outcome and potential outcomes are defined as per unit.  In relational settings the entities to which a treatment applied to or withheld from are often different from entities over which an outcome of interest is measured. This make the identification of the units of causal analysis challenging.  For example, in analysing the effect of the teaching skill of instructors on student performance, depending on the outcome on interest, students, classrooms, instructors, and even the combination of students and classes would be the appropriate units of analysis.  For instance, if the outcome is average of students grade in classes teach by an instructor, then the potential outcome must be defined as per instructor, hence instructors would be the units of analysis. However, for the outcome of student grade the students serve as units of analysis. Indeed, the choice of unit would affect the range of causal queries that could be supported.
% 
The POF also relies on an ariori assumption called SUTVA that states the value of $Y$ for unit $u$ when exposed to treatment  $t$ will be the same no matter what mechanism is used to assign   treatment $t$ to unit $u$ and no matter what treatments the other   units receive $\forall t \forall i$.  Violations of SUTVA if the units {\em interfere} ...

Most of the literature on causal inference in the presence of interference developed within the {\em potential outcome framework} (POF) (cf. Sec~\ref{sec:causal-framework}),  These works are not immediately applicable to relational domains because of the following methodological challenges.   In relational settings a unit may subject to a {\em multidimensional treatment} vector. For example, to study the effect of tutoring on GPA of a student, the treatment of a student is a multi-dimensional vector of treatment assigned to each classes enrolled by the student. Presence of multidimensional treatments create new challenges that have not been studied in the literature. In addition,  the existing work in causal inference are typically interested in evaluating the effects of a treatment that can be applied {\em individually} on the experimental units. However, in relational settings, a treatment frequently applied to a group of entities that are relationally connected. For example. in analysing an educational intervention, treatment may be applied to classrooms of student.  In such, scenarios the treatments of individual units becomes {\em entangled}, which makes causal inference challenging \cite{toulis2018propensity}.


%
%Now, if the goal of analysis is to the effect of treatment on an outcome measured for each individual, e.g., student grade, the potential outcome must be defined as per each student, hence students serve as unit.

%Furthermore, in relational setting, the entities that received treatment and entities 




%A basic concept, in potential outcome framework for causal inference,  In causal inference, a causal query concerned about the effect of assigning a treatment level (an intervention) to an {\em ``experimental unit"}, e.g., person, patience, organisations, on a response variable measured on an {\em``observational unit"} that could be different than the experimental unit. 


%The existing work in causal inference typically interested in setting in which the treatments can be {\em individually} applied to experimental units and observational and experimental units are the same. For example, in a medical trials,  patients are serve both as experimental and observational units. In contrast, in relation settings, a treatment frequently applied to a group of experimental units that are relationally connected. Moreover, experimental and observational units are often different. For example, in the university domain, to study the effect of tutoring on students grade, the treatment of tutoring applied to classrooms as oppose to individual student. hence the treatment of each individual student are {\em entangled} \cite{toulis2018propensity}. Alternatively, one might regard class room as experimental units.  Moreover, the measurement of progress obtained on each individual student. 

%Identifying the experimental and observational units is a key step for expressing causal queries. In this section, we show RelCMs provide a convenient formalism for expressing causal queries and identifying units of an analysis in natural and implicit manner.  

%However, in relational settings


%\section{Related Work}




==> TODO.tex <==
\section{Discussion and Related Work}
\label{sec:discussions}



==> implementation.tex <==


\section{System and Implementation}\label{sec:overview}
\red{[Outdated]}

The system is composed of four main components, illustrated in Figure \ref{fig:overview}. 

\paragraph{Normalization module}
The unit accepts \rcr s and is responsible for rewriting the query such that only fixed-arity rules remain. It also emits the list of embeddings that the relational unfolding module must learn to account for the adjusted structure.

\paragraph{Covariate and treatment detection} This accepts a query and is responsible for selecting the relevant covariates from the normalized graph provided by the first module. It is also responsible for identifying treatment atoms. The output of this module, along with that of the normalization module, is passed to the \textit{relational unfolding module}.

\paragraph{Relational unfolding module} This learns the requisite unfoldings, given the relevant covariates and possible embeddings. It then caculates those unfoldings, and so module produces a flat table, which is passed to the \textit{estimation module}.

\paragraph{Estimation module} This is an off-the-shelf component that calculates the final output: an estimate of the causal effect.


\red{DISCUSS TOP K from 4.2.5}





==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

% lg1 - overall, I think we want to minimize jargon used
% e.g., why do we have to talk about generative models here,
% also, there is so much very basic stuff here, but then
% there is not a road madp that helps to say what is coming in terms of what is stuff that exists that we use
% versus what is new.   some how getting ready for the hard part.
% also, maybe now I've gotten too used to causal, but acknowledging
% that it's a big thing, everyone thinks it's important, etc.
% 

% lg1 - is there a way to structure this so that it includes the acknowledgement that
% there is growoing body of work that addresses 
% aka, there are too many points trying to be made here -- is it causal vs. associational? or 
% causal vs relational causal?   I think we want the latter
%
% lg1 - original below

% lg1 - decide on which terms are absolutely required to be defined here, and only define them
%
% terms left out: generative, associational, predictive analytics

The importance of causal reasoning for making informed policy
decisions has long been recognised in healthcare, medicine, social
sciences, and other domains. 
%However, today's machine learning systems
%typically do not go beyond {\em predictive analytics} and thus fail to
%answer questions such as 
%``What will happen to revenue if the price of
%X is lowered?'' 
%While predictive analytics has achieved remarkable
%success in diverse applications, it is mostly restricted to fitting a model to
%observational data based on {\em associational}
%patterns~\cite{pearl2018book}.} %
%on the other hand,
%goes beyond associational patterns to the process that generates the
%data, 
Causal inference enables analysts to reason about {\em interventions}  (e.g. ``Would requiring flu shots in schools reduce the chance of a future flu epidemic?") and {\em counterfactuals} (e.g. ``What would have happened if past flu shots were not taken?"). 
The gold standard in causal analysis is performing {\em randomized control trials}, where the {\em subjects} or {\em units} of
study are assigned randomly to a treatment or a \revm{control (i.e., withheld
from the treatment) group}.  
% lg1 - do we need average treatment effect defined here?
%The difference between the average of the outcome variable of
%the treated and control groups is called the \emph{average
 % treatment effect}, and represents the causal effect. 
Unfortunately
controlled experiments are not always feasible due to ethical, legal,
or cost constraints. 
An attractive alternative that is receiving growing attentions in the 
statistics, economics, and social sciences simulates controlled
experiments using {\em observational studies} on available data.  While we can no longer assume that
the treatment has been randomly assigned, under appropriate
assumptions we can still \cutr{learn causal relationships.}
\revm{estimate causal effects.} \revm{
Rubin's Potential
Outcome Framework~\cite{rubin1970thesis} and Pearl's Causal
Models~\cite{PearlBook2000} (reviewed in Section~\ref{sec:background}) are
two popular frameworks  for observational causal analysis.
}

Both of these causal frameworks rely on the critical assumption that
the units of study are sampled from a population of homogeneous units;
in other words, the data can be represented in a single flat table.  In many real-world
settings, however, the study domain consists of {\em heterogeneous units} that
have a {\em complex relational structure}; and the data is naturally represented as multiple related tables.
Furthermore, reasoning about dependencies between units is important -- for example, 
\lise{to do, expand with english description of the problem....}

% lg1 - I find the movating example too dense to include in the intro.   I suggest move it out, into it's own section.   I know this pays a price in terms of space, but I think it is worth it
In this paper, we develop new theory and methods for causal inference in relational domains.    Our
work builds upon existing work in causal modeling \cite{pearl2014probabilistic} and relational learning \cite{rellearning}, and we
validate our framework on several real-world and synthetic domains.
%
% lg1 - can we try to remove some to the vocabulary here, and not overload readers with 
%\vspace{-2mm}
%\textbf{Our contributions.~}  
We propose a declarative framework for {\em Causal
  Relational Learning} \cutr{a foundation for} 
 \revm{to support} causal inference over
\revm{relational data stored in multiple inter-related tables}. %domains. 
Our first contribution is a declarative language, \emph{\sys\ (Causal Relational Language)}, for representing causal background knowledge and assumptions \cutr{in relational domains} 
\revm{for relational data} ({\bf Section~\ref{sec:causal-framework}}). 
\sys\ can represent complex \revm{\emph{causal models}, i.e., potential causal dependence among the units}  using \cutr{just a few}
\revm{intuitive declarative} rules.  Given a database
instance\cut{(which we call a {\em skeleton})}, these rules are then
grounded to form a large ground causal graph, consisting of heterogeneous
units with complex inter-relationships.  \cut{To use the ground 
causal graphs for causal inference,
we make an important {\em structural homogeneity} assumption, which states that ground atoms of the same
type share the same {\em structural equations}; in other words, they share the same generative process.  Furthermore,} \revm{Most importantly,} details of the semantics of causal models are abstracted from the users, who \cutr{no longer}
\revm{do not} need to be statisticians;  instead, they can write {\em causal queries} in a high-level declarative language. \revm{We discuss the extensions in \sys\ over previous work in detail after we review the basic concepts and literature in causal analysis in Section~\ref{sec:background}.}
\par
Our second contribution
is a non-trivial extension of Pearl's $\Do$-operator to give semantics to complex causal queries about the \revm{average treatment effect}, and \emph{isolated}, \emph{relational}, and \emph{overall} effects of interventions ({\bf Section~\ref{sec:semantics}}).  When investigating the effect of authors' prestige on review scores (Example~\ref{ex:univdomain:causalmodel}), \revm{the isolated and relational effects respectively  measure to what extent the review scores are influenced by an author's own prestige
%. The relational effect measures to what extent the review scores of an author are influenced
and by the prestige of his or her collaborators}. We show that the overall effect is the sum of isolated and relational effects. 


% However, using \sys\ the users can pose these queries declaratively without
%without the need to know how these queries are mapped to the grounded causal model.
%The $do$-operator is defined as an
%intervention on one (or several) variables in a causal model.  In \sys,
%Our semantics defines how
%to map those treatments to $do$-operators on the grounded causal DAG.
\par
Our third contribution consists of an algorithm for answering 
causal queries from the given relational data ({\bf Section~\ref{sec:causal-queries:answering}}).  \revm{The algorithm detects a set of confounding covariates for a causal query given a causal graph and then makes relational causal analysis amenable to existing approaches by constructing a single unit table by embedding vectors of treatment, response, and covariates to smaller dimensions.}
\cutr{performs a static analysis of the causal query, and it constructs a unit-table specific to
the query and the relational causal model by identifying a set of attributes
that are sufficient for confounding adjustment.}   
\par
Finally, we present an end-to-end experimental evaluation of \sys\ ({\bf Section~\ref{sec:experiments}}) on %both
\revm{three real datasets -- \data\ \cite{OpenReview, scopus, shanghai} (an integrated review dataset as in Example~\ref{ex:univdomain:causalmodel},  \mimicdata\ \cite{mimic} (the Multiparameter Intelligent Monitoring in Intensive Care dataset, and \nisdata\ \cite{healthcare_cost_and_utilization_project_hcup_hcup_2006} (the Nationwide Inpatient Sample dataset)}), as well as on synthetic \data. 
%real and synthetic data 
We find that causal queries indeed provide quite different insights over real data compared to simple
associational queries that compute correlations, or compared to a naive causal analysis that
assumes homogeneous units and ignores relationships.  Over synthetic data (for which the ground truth is known),  \sys\ was
able to recover the ground truth. \revm{Over the real datasets, \sys\ found interesting answers for the following causal queries: (1) What is the effect of institutional prestige on reviewers' recommendations under single-blind and double-blind review processes? (2) What is the effect of not having insurance on patient mortality and length of stay? (3) What the effect of hospital size on affordability of healthcare?}




% 
\section{Motivating example}



\cut{
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{Figures/obs.pdf}
    \caption{Number of publications that include observational studies
      vs controlled experiments (obtained from
      SemanticScholar~\cite{SemanticSchoolar}).
      %\dan{(1) the figure  takes too much area compared to how much information it  conveys.  Can we make it shorter (and also wider, since there   is unused space at the margins)?  (2) please increase the fonts; also you can remove some of the labels on the Oy axis,    e.g. it suffices to show 2-4-60000, or even less.}
      }
    \label{fig:obstrend}
\end{figure}
}

Lead with an explanation of what the domain is, etc. there's alot of the writing that is about the data set; the point of the example is only to illustrate the idea.   so tighten, move details to end or appendex, and 
write this only as an example.

soemthing more like
Consider the following domain describing authors and publications (see fig).
Supposed we are interested in answering the question of xxxx?
THis is relational because yyyyy



\begin{example} (\data) \em \label{ex:univdomain:causalmodel}
  OpenReview~\cite{OpenReview} is a collection of paper submissions from several conferences, mostly in ML and AI, along with their reviews. \revd{The collection contains review scores and author information for both
  accepted and rejected papers.}  Scopus~\cite{scopus} is a large, well
  maintained database of peer-reviewed literature, including
  scientific journals, books and conference proceedings. The Shanghai University Ranking~\cite{shanghai} is one of three authoritative global university rankings.  We crawled
  and integrated these sources to produce a relational database,
  which we show in simplified form in
  Figure~\ref{fig:example_instance}.  Data sources like this represent a
  treasure trove of information for the leadership of scientific
  conferences and journals.  For example, they can help answer
  questions like ``Does double-blind reviewing achieve its desired effect?'' or
  ``Does increasing (or decreasing) the page limit affect paper quality, and if so, how?''.  To answer these real-life questions,
  discovering association is not sufficient; instead, decision
  makers need to know if there exists a causal effect. For
  example, suppose a conference is currently requiring double-blind
  submissions, and the leadership is questioning the effectiveness of this policy.  If leadership reverts to single-blind submissions, would that represent an
  unfair advantage for authors from prestigious institutions? 
%\dan{don't overcomplicate it.  We have already given two examples  above, now we need to narrow down to the question the we will  eventually answer in the experiments.  Whether it's about prestige of authors or prestige of institutions, that's exactly how we should formulate the question here.}
  Given  a dataset like that in Figure~\ref{fig:example_instance}, one can run a few
  SQL queries and check whether those authors consistently get better
  reviews at single- rather than double-blind
  venues. However, this only proves or disproves correlation, 
  not causation.  Alternatively, one could apply Rubin's Potential Outcome Framework~\cite{rubin1970thesis, rubin2005causal}, but that requires 
  data to be presented as a single table of independent units.  Doing this
  naively on our dataset (\eg, computing the universal
  table~\cite{ullm82}) means one cannot account for \revm{various ``interactions'' among the entities of interests.}
  %that prohibit standard causal analysis.} 
  \cutr{what statisticians refer to as {\em interference}  and
  {\em contagion} effects~\cite{tchetgen2012causal, ogburn2014causal},   both of which prohibit standard causal
  analysis. } %\babak{joining data sets do not create  contagion and interference, these are properties of the data
   %generative model (how the %domain works)}
  %\dan{you are right.  But the point to make here is that the
   % relational data captures correctly the generative model, but if we
    %just join them and re-define units based in the joint data, then
    %there is intereference and contagion. Do you agree?}
For instance, the prestige of an author not only influences
  his or her acceptance rate, but it also has a {\em spill-over} effect on the acceptance rate of  his or her co-authors; this is called interference.
  Further, authors' qualifications can be {\em contagious}, meaning that if a junior author collaborates frequently with a
  senior author, then the overall quality of his or her own research may
  increase over time.
    \revm{To our knowledge, no tools exist that can model and address such intricate dependencies while allowing sound causal analysis accessible to a broad range of  data analysts.}
  \end{example}
  
  %\revm{Target audience of the relational causal learning }


  %\red{SR: WRITE A FEW LINES ABOUT OTHER DATASETS AND EXMAPLES.}
%   shows a simplified scheme of a
%   relational data we crawled from publicly available
%   websites~\cite{OpenReviwe,scopus}. The schema consists of the
%   entities $\mathit{People}$, $\mathit{Conference}$ and
%   $\mathit{Submission}$; and their relationships $\mathit{Author}$ and
%   $\mathit{Submitted}$; and a set of descriptive attributes such as
%   $\mathit{Decision}$ (whether a submission is accepted or rejected),
%   $\mathit{Blind}$ (whether a conference uses single or double-blind
%   reviewing) and $\mathit{Prestige}$ (whether an authors is afflicted
%   with a high-prestige institution). An interesting question that can
%   be investigated using \data\ is whether single-blind reviewing
%   confers any advantage to submissions from authors with high-prestige
%   institutions.  Specifically, we are interested in computing the
%   causal effect of authors' prestige on paper's decision. Note that
%   institutional prestige is perceived to be a significant predictor
%   for paper acceptance, thereby predictive analysis can be
%   perplexing. Additionally, this is challenging, as we are facing a
%   relational domain consisting of related heterogeneous
%   entities. Here, the institutional prestige belongs to the
%   $\mathit{Author}$ table, whereas the decision of a submission belong
%   to the $\mathit{Submission}$ table. Therefore, we don't have a unit
%   of study in in the sense of Rubin \cite{rubin1970thesis}. This rules
%   out using Rubin's causality out-of-the-box.  Furthermore, this
%   relational domain has a complex causal structure in which entities
%   exhibit {\em interference} and {\em contagion}. For instance,
%   prestige of an author not only influences their acceptance rate, but
%   also has a {\em spill-over} effect on the acceptance rate of their
%   co-authors, hence authors interfere. Moreover, authors
%   qualifications can be {\em contagious} over a course of
%   time. However, Pearl's causality does not permit us to describe such
%   complex relational causal dependencies between {\em multiple}
%   heterogeneous entities in a succinct way.
% 



\begin{figure}
    \centering
    \input{instance.tex}
    \caption{%\vspace{-2mm}
%    \lise{I accidently deleted,:(}
\red{Fragment of schema and toy instance for XXX.
    }}
     \vspace{-0.5cm}
    \label{fig:example_instance}
\end{figure}

\cut{
\vspace{-2mm}
\textbf{Our contributions.~}  In this paper, we propose a declarative framework for {\em Causal
  Relational Learning} \cutr{a foundation for} 
 \revm{to support} causal inference over
\revm{relational data stored in multiple inter-related tables}. %domains. 
Our first contribution is a declarative language, \emph{\sys\ (Causal Relational Language)}, for representing causal background knowledge and assumptions \cutr{in relational domains} 
\revm{for relational data} ({\bf Section~\ref{sec:causal-framework}}). 
\sys\ can represent complex \revm{\emph{causal models}, i.e., potential causal dependence among the units}  using \cutr{just a few}
\revm{intuitive declarative} rules.  Given a database
instance\cut{(which we call a {\em skeleton})}, these rules are then
grounded to form a large ground causal graph, consisting of heterogeneous
units with complex inter-relationships.  \cut{To use the ground 
causal graphs for causal inference,
we make an important {\em structural homogeneity} assumption, which states that ground atoms of the same
type share the same {\em structural equations}; in other words, they share the same generative process.  Furthermore,} \revm{Most importantly,} details of the semantics of causal models are abstracted from the users, who \cutr{no longer}
\revm{do not} need to be statisticians;  instead, they can write {\em causal queries} in a high-level declarative language. \revm{We discuss the extensions in \sys\ over previous work in detail after we review the basic concepts and literature in causal analysis in Section~\ref{sec:background}.}
\par
Our second contribution
is a non-trivial extension of Pearl's $\Do$-operator to give semantics to complex causal queries about the \revm{average treatment effect}, and \emph{isolated}, \emph{relational}, and \emph{overall} effects of interventions ({\bf Section~\ref{sec:semantics}}).  When investigating the effect of authors' prestige on review scores (Example~\ref{ex:univdomain:causalmodel}), \revm{the isolated and relational effects respectively  measure to what extent the review scores are influenced by an author's own prestige
%. The relational effect measures to what extent the review scores of an author are influenced
and by the prestige of his or her collaborators}. We show that the overall effect is the sum of isolated and relational effects. 



% However, using \sys\ the users can pose these queries declaratively without
%without the need to know how these queries are mapped to the grounded causal model.
%The $do$-operator is defined as an
%intervention on one (or several) variables in a causal model.  In \sys,
%Our semantics defines how
%to map those treatments to $do$-operators on the grounded causal DAG.
\par
Our third contribution consists of an algorithm for answering 
causal queries from the given relational data ({\bf Section~\ref{sec:causal-queries:answering}}).  \revm{The algorithm detects a set of confounding covariates for a causal query given a causal graph and then makes relational causal analysis amenable to existing approaches by constructing a single unit table by embedding vectors of treatment, response, and covariates to smaller dimensions.}
\cutr{performs a static analysis of the causal query, and it constructs a unit-table specific to
the query and the relational causal model by identifying a set of attributes
that are sufficient for confounding adjustment.}   
\par
Finally, we present an end-to-end experimental evaluation of \sys\ ({\bf Section~\ref{sec:experiments}}) on %both
\revm{three real datasets -- \data\ \cite{OpenReview, scopus, shanghai} (an integrated review dataset as in Example~\ref{ex:univdomain:causalmodel},  \mimicdata\ \cite{mimic} (the Multiparameter Intelligent Monitoring in Intensive Care dataset, and \nisdata\ \cite{healthcare_cost_and_utilization_project_hcup_hcup_2006} (the Nationwide Inpatient Sample dataset)}), as well as on synthetic \data. 
%real and synthetic data 
We find that causal queries indeed provide quite different insights over real data compared to simple
associational queries that compute correlations, or compared to a naive causal analysis that
assumes homogeneous units and ignores relationships.  Over synthetic data (for which the ground truth is known),  \sys\ was
able to recover the ground truth. \revm{Over the real datasets, \sys\ found interesting answers for the following causal queries: (1) What is the effect of institutional prestige on reviewers' recommendations under single-blind and double-blind review processes? (2) What is the effect of not having insurance on patient mortality and length of stay? (3) What the effect of hospital size on affordability of healthcare?}
}

\cutr{\data, we present interesting findings on the causal effect of prestige on submission scores in single- versus double-blind venues. \red{SR: UPDATE AFTER OTHER EXPTS.}}

% In this paper, we propose a declarative framework for {\em Causal
%   Relational Learning}, a foundation for causal inference over
% relational domains. Specifically, we propose a declarative language, which allows us to define a {\em Relational Causal Model} for representing causal relationships between heterogeneous units, with
% complex relational structures, then allows us to formulate {\em Causal
%   Queries} over a given relational database, by using the same
% high-level declarative language.  We give semantics to the causal
% queries by proposing a new, non-trivial extension of Pearl's
% $\Do$-operator to relational causal models.  We then propose an
% algorithm for evaluating causal queries from the given data, by
% creating on-the-fly a table of units (specific to the query) and
% finding a sufficient set of {\em covariates} that should be adjusted
% for to remove confounding effects. 
% %%% We formalize complex causal queries about isolated and relational
% %%% effects in multi-relational settings. We propose techniques such
% %%% as {\em embedding relational data} for transforming relational
% %%% data into a flat table amenable for easy causal inference.
% Finally, we conduct an experimental evaluation of \sys\ on both real
% and synthetic data.  We make the following specific contributions.
 
 
%\dan{I think that this paragraph still needs work to explain our  contributions} \babak{revised} \dan{Sorry, it's still wasn't what it needs to be; here we need to brag about {\em our} system, and our system only.  I commented out the old paragraph in Latex, and replaced with this new one.  Please update: it is too long, and I probably did not capture well the contributions in Sections~\ref{sec:causal-query} and ~\ref{sec:causal-queries:answering}.  This paragraph needs to be written such that an expert reader can understand it, and appreciate it.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%DAN'S
%Our first contribution is a declarative language, \emph{\sys\ (Causal Relational Language)}, for representing casual background knowledge and assumptions in relational domains.  The language can define complex causal models in relational domain using just a few rules.  Given a databaseinstance (which we call a {\em skeleton}), these rules are then
%grounded to form a large ground causal graph, consisting of heterogeneous
%units with complex inter-relationships.  In order to learn thestructural equations from the given data because, we make an important
%{\em homogeneity assumption}, by assumeing that all nodes of the same
%type have the same structural equations; in other words, nodes of the
%same type are governed by the same laws of physics.  Users do not need
%to be aware of the causal DAG, but instead write {\em causal queries}
%in the high-level declarative language.  Our second contribution
%consists of a non-trivial extension of Pearl's $Do$-operator to give
%semantics to these queries.  The $do$-operator is defined as an
%intervention on one (or several) variables in a causal DAG.  In \sys,
%however, the user asks causal queries in a declarative language, where
%the treatments are specified declaratively.  Our semantics defines how
%to map those treatments to $do$-operators on the grounded causal DAG.
%Our third contribution consists of an algorithm for answering the
%causal queries from the given data.  The algorithm performs a static%
%analysis on the causal query, and constructs a unit-table, specific to
%that query and the relational causal model, then finds the covariates,
%and computes the average treatment effect.  Finally, our fourth
%contribution consists of an experimental evaluation of \sys\ on both
%real data and synthetic data.  We find that causal queries provide
%indeed quite different insights over the real data than simple
%associational queries, or even than a naive causal analysis that
%assumes homogeneous units and ignores relationships.  We also found
%that, over synthetic data (where we had the ground truth) \sys\ was
%able to recover the ground truth with good accuracy.



%, then finds the covariates,
%and computes the average treatment effect.

%%% At the core of relational causal models is a declarative language that
%%% allows users to specify assumptions and background knowledge on the
%%% causal interactions among heterogeneous units, and to formulate causal
%%% queries. As oppose to predictive analysis, domain expert knowledge
%%% plays a critical role and is fundamentally required for causal
%%% inference \cite{pearl2009causal}. Pearl proposed causal graphs as a
%%% powerful mathematical tool for specifying these background
%%% knowledge. \footnote{The use of graphical models for capturing causal
%%%   relationships can be traced back to Sewall Wright's introduction of
%%%   path diagram in the early 1920~\cite{wright1921correlation}}
%%% However, as we argue in Section~\ref{sec:background} causal graphs are
%%% incapable of capturing causal relationships in complex relational
%%% domains in which heterogeneous units exhibit interference and
%%% contagion, e.g., the effect of collaborators of a professor on their
%%% student' learning. In contrast, in our declarative language called
%%% \sys\, users can specify complex background knowledge and their causal
%%% queries about relational domains with simple and intuitive
%%% Datalog-like rules.
%%% 

\cut{
In summary, we make the following contributions.  (1) We propose
Relational Causal Models with a declarative language
(Sec.~\ref{sec:causal-framework}).  (2) We introduce the semantics of
causal queries by extending the $do$-operator
(Sec~\ref{sec:causal-query}), (3) We develop a query answering
algorithm (Sec.~\ref{sec:causal-queries:answering}) and (4) we conduct
an experimental evaluation (Sec.~\ref{sec:experiments}).
}

%%% \dan{We should have one contribution per section.}  We make the
%%% following contributions: (1) We propose Relational Causal Molds, which
%%% lift Pearl's Causal Models to relational domains. (2) We propose \sys\
%%% a declarative language for capturing users’ assumptions and queries
%%% using simple Datalog-like rules. (2) We develop an underlying
%%% inference engine that automatically detects a sufficient set of {\em
%%%   covariates} that should be adjusted for to remove confounding
%%% effects. (3) We develop novel techniques such as {\em embedding} to
%%% transform relational data into a flat table amenable to easy causal
%%% inference.  (4) we answers a suite of causal queries considering
%%% relational and isolated effects. (5) We evaluate \sys\ on synthetic
%%% and real data, and illustrate the applicability of our method on
%%% estimating the causal effect of institutional prestige on the
%%% acceptance of papers under single-blind and double-blind review
%%% processes.
%%% 


%
%In this paper we develop the theory of {\em Relational Causal Models}, or ReCMs; grounded in Pearl's causal model  ReCMs provide a foundation for inferring causal inference from relational domain. ReCMs lift
%Pearl's causal models from representing causal relationship between attributes of homogeneous units, to heterogeneous units that are related with complex relational dependencies.  We extend Pearl's  $\Do$-operator to ReCMs, to capture complex interventions in relational domains.
\vspace{0.1cm}




%notion of causality studies in this paper is fundamentally different from prior works in query answer causality and responsibility and explanation \cite{RoyS14} and hypothetical reasoning  \cite{balmin2000hypothetical,lakshmanan2008if, deutch2013caravan} which aims to identify parts of the input that are correlated with query answers.  









%\sys\ extends the existing literature  (3) ground in the existing framework in causal inference, \sys\ articulate the assumptions required for making causal inference from relational data.



%to model a joint probability distribution over relational data amenable for probabilistic reasoning rather than causal inference ~\cite{Getoor:2007:ISR:1296231}.  However, using a causal interpretation of these dependency models in statistical relational learning, called {\em Relational Causal Graphical Models}, the authors in \cite{arbour2016inferring} studied interference in the context of social 

%{\em directed acyclic probabilistic entity-relationship} (DAPER)  \cite{heckerman2007probabilistic}.


% 
%\babak{add the work on homophily}

%Statistical Relational Learning (SRL) aims at unifying logic and probability to model a joint probability distribution over relational data amenable for probabilistic reasoning~\cite{Getoor:2007:ISR:1296231}. A plethora of models such as PRMs \cite{getoor2007probabilistic}, PSL, DAPER, PBNs, BLPs and MLNs has been proposed for SRL in the literature.  While our proposed framework for Causal Relational Learning, \sys, shares some similarities with some of these models, it is fundamentally motivated for causal reasoning. The closest SRL model to \sys\ are PRMs and  DAPER that extend the standard entity-relationship (ER) model to incorporates probabilistic dependencies. They can also be seen as a first-order extension of Bayesian Networks to relational data. However, there are two primary differences between \sys\ and these models. First, PRMs are dependency models that essentially define a joint probability distribution over all possible completions of a partially specified instance. In contrast \sys\ models the generative process of relational data. Here, the uncertainty is induced by hidden noise variables, {\em and prevails even
%when the entire relational data is available}. There has been prior attempt to 
%use use these models for causal inference from relational data, e.g., 


%At the core of ReCMs is a declarative language that can capture complex causal structure that are present in real-world scenarios and an inference ..





%that allows complex relational data to be mapped to the standard model used in statistics to perform causal inference. Using new techniques such as {\em embedding relational data}, RCMs can efficiently answer complex causal queries about the {\em interference} and {\em spill-over effect} of treatment strategies.




%in which the treatment is to instruct authors to manipulate their name/affliction in their submissions and the outcome is the submission's decision. 
%relational domain is challenging.  First, the domain consists of heterogeneous entity classes such as $\mathit{Author}$,  $\mathit{Submission}$ and  $\mathit{Conference}$ that are interconnected with relational dependencies (See Fig~\ref{fig:erdiagram}). Therefore, the units that receive a treatment can be different than the unit for which an outcome of interest in measured. In our case, the treatment of prestige applied to or withheld from each author, but response of decision measured for each submission. This rules out using Rubin's POF out-of-the-box. Furthermore, the treatment of  prestige of one author would affect the acceptance rate of all of his co-authors


%Presumably, authors from prestigious universities are submitting high-quality work, hence prestige is a {\em significant predictor} for acceptance, even when they are {\em causally independent}.


%This rules out using Rubin's POF out-of-the-box.

%Now, the 
 %Hence, even in double-blind reviewing we expect  author's prestige to be a significant predictor for paper acceptance.

%we expect a huge correlation between authors prestige 
%The entity-relationship diagram in Fig~\ref{fig:erdiagram} represents a simplified academic conference domain consist of three entity classes  $\mathit{Author}$,  $\mathit{Submission}$ and  $\mathit{Conference}$. Each author may have several submissions; and vice versa a submission may have several authors. A conference may receive several submissions, but each submission only associated to one conference. The attributes $\mathit{Impact}$, $\mathit{Productively}$ and $\mathit{Experience}$ describe the qualifications of the authors. $\mathit{Prestige}$ shows the prestige of the institution the authors are affiliated with. The attribute $\mathit{Quality}$ and $\mathit{Decision}$  respectively shows whether the submission has a decent quality and whether is it has been accepted or rejected for publication. 
%Finally, $\mathit{Blind}$ shows whether a conference follows a single vs double blind review policy.



%here is a many-to many relationship between  $\mathit{Author}$ and submissions and a one-to-many relationship between a $\mathit{Conference}$ and $\mathit{Submission}$.

%Consider the the causal graph in Fig~\ref{fig:dag:univer} representing a potential causal relationships in the paper authorship and scientific peer-review scenario. 

%The graph postulates the following causal relationship:
%\begin{itemize}
%    \item ``Prestige" of an author for a paper is dependent on the number of citations, experience and productivity of the author.
%    \item ``Quality" of the paper is also a function of citations of the authors and their experiences. The contribution of each author's covariates depends on their position in the list of authors for a given paper.
 %   \item ``Review-score" assigned by the group of reviewers to a paper submitted to a conference is dependent on the quality of the paper, rigor of the conference while it is hypothesized to depend on the prestige of the authors for single-blind venues. 
%\end{itemize}




%However, the causal DAG fails to capture confounding due to causal interaction of objects from related entities. For instance, to assess the effect of prestige of the author on review score of the submission one need to account for the authors' colleagues who the authors have worked with in the past as it might affect author's prestige.\harsh{here!} As shown in Fig~\ref{}(b), this example has: 1) \textit{interference}, because the tutoring received by one students affects the peer's outcomes; 2) \textit{contagion}, because related students are likely to study together and hence their outcomes affect each other's outcomes; and 3) \textit{induction}, because student tend to choose course which their friends choose and hence the treatment choice of one affects other's choice. Expressing causal interaction between the related objects in a network using non-structural equations (NSEs) is either impossible or tedious. 

%Our major contribution in this paper is the introduction {\em relational causal models}. We propose a richer language to describe {\em relational causal models} and an inference methodology which can capture complex causal dependencies that are present in real-world scenarios. The goal is to provide the theoretical foundation and tools for answering the following types of causal queries in relational settings:
%\begin{itemize}
   % \item What is the effect of tutoring sections on the grades of a student in a class?
  %  \item What is the effect of tutoring on the attendance rate of the student in that course?
   % \item what is the effect of one's lecture attendance in a class on one's grade in that class?
   % \item What is the effect of having team projects on the average grade in the class?
%\end{itemize}



==> introduction3.tex <==
\section{Introduction}
\label{sec:intro}

The importance of causal inference for making informed policy
decisions has long been recognised in health, medicine, social
sciences, and other domains. However, today's decision-making systems
typically do not go beyond {\em predictive analytics} and thus fail to
answer questions such as ``What will happen to revenue if the price of
X is lowered?'' While predictive analytics has achieved remarkable
success in diverse applications, it is mostly restricted to fitting a model to
observational data based on {\em associational}
patterns~\cite{pearl2018book}. Causal inference, on the other hand,
goes beyond associational patterns to the process that generates the
data, {thereby enabling analysts to reason about {\em interventions}  (e.g. ``Would requiring flu shots in schools reduce the chance of a future flu epidemic?") and {\em counterfactuals} (e.g. ``What would have happened if past flu shots were not taken?").} \revm{This adds significantly more information in data analysis compared to simple correlation or regression analysis; e.g., with more flu cases, the rate of taking flu shots might increase, but that does not imply that taking flu shots  increases the spread of flu. This emphasizes the %well-known nugget of wisdom 
common saying that ``correlation is not causation'', which is known to all, but is easy to overlook if one is not careful while analyzing data for insights and possible actions.}

The gold standard in causal analysis is performing {\em randomized
  controlled experiments}, where the {\em subjects} or {\em units} of
study are assigned randomly to a treatment or a \revm{control  (i.e., withheld
from the treatment) group}.  The difference between the average of the outcome variable of
the treated and control groups is called the \emph{average
  treatment effect}, and represents the causal effect. However,
controlled experiments are not always feasible due to ethical, legal,
or cost constraints. An attractive alternative that has been used in
statistics, economics, and social sciences simulates controlled
experiments using {\em observational studies} on available data.  While we can no longer assume that
the treatment has been randomly assigned, under appropriate
assumptions we can still \cutr{learn causal relationships.}
\revm{estimate causal effects.} \revm{Two %well-
established frameworks  for observational causal analysis, %exist for this purpose 
Rubin's Potential
Outcome Framework~\cite{rubin1970thesis} and Pearl's Causal
Models~\cite{PearlBook2000} (reviewed in Section~\ref{sec:background}),
have been  extensively studied %and applied 
in the literature of statistics, artificial intelligence,
social science, health, 
and other application domains.}


 Causal frameworks, however, rely on the critical assumption that
the units of study are sampled from a population of homogeneous units;
in other words, the data can be represented in a single flat table.  In many real-world
settings, however, the study domain consists of {\em heterogeneous units} that
have a {\em complex relational structure}; and the data is naturally represented as multiple related tables. \revm{For instance, as presented later in our experiments with real data \cite{mimic, healthcare_cost_and_utilization_project_hcup_hcup_2006}, %\red{SR: CITE NIS},  
hospitals can record   in several tables information about patients, medical practitioners, hospital stays, treatments performed, insurance, bills, and so on. }  Standard
notions used in causal analysis --- such as \revm{units or subjects who receive a treatment in causal analysis} ---
%,  covariates and casual graphs --- 
no longer \revm{readily} apply to relational data, prohibiting us from adopting existing causal inference frameworks to relational domains.
We illustrate these challenges with an example.
\vspace{-2mm}
\begin{example} (\data) \em \label{ex:univdomain:causalmodel}
  OpenReview~\cite{OpenReview} is a collection of paper submissions from several conferences, mostly in ML and AI, along with their reviews. \revd{The collection contains review scores and author information for both
  accepted and rejected papers.}  Scopus~\cite{scopus} is a large, well
  maintained database of peer-reviewed literature, including
  scientific journals, books and conference proceedings. The Shanghai University Ranking~\cite{shanghai} is one of three authoritative global university rankings.  We crawled
  and integrated these sources to produce a relational database,
  which we show in simplified form in
  Figure~\ref{fig:example_instance}.  Data sources like this represent a
  treasure trove of information for the leadership of scientific
  conferences and journals.  For example, they can help answer
  questions like ``Does double-blind reviewing achieve its desired effect?'' or
  ``Does increasing (or decreasing) the page limit affect paper quality, and if so, how?''.  To answer these real-life questions,
  discovering association is not sufficient; instead, decision
  makers need to know if there exists a causal effect. For
  example, suppose a conference is currently requiring double-blind
  submissions, and the leadership is questioning the effectiveness of this policy.  If leadership reverts to single-blind submissions, would that represent an
  unfair advantage for authors from prestigious institutions? 
%\dan{don't overcomplicate it.  We have already given two examples  above, now we need to narrow down to the question the we will  eventually answer in the experiments.  Whether it's about prestige of authors or prestige of institutions, that's exactly how we should formulate the question here.}
  Given  a dataset like that in Figure~\ref{fig:example_instance}, one can run a few
  SQL queries and check whether those authors consistently get better
  reviews at single- rather than double-blind
  venues. However, this only proves or disproves correlation, 
  not causation.  Alternatively, one could apply Rubin's Potential Outcome Framework~\cite{rubin1970thesis, rubin2005causal}, but that requires 
  data to be presented as a single table of independent units.  Doing this
  naively on our dataset (\eg, computing the universal
  table~\cite{ullm82}) means one cannot account for \revm{various ``interactions'' among the entities of interests.}
  %that prohibit standard causal analysis.} 
  \cutr{what statisticians refer to as {\em interference}  and
  {\em contagion} effects~\cite{tchetgen2012causal, ogburn2014causal},   both of which prohibit standard causal
  analysis. } %\babak{joining data sets do not create  contagion and interference, these are properties of the data
   %generative model (how the %domain works)}
  %\dan{you are right.  But the point to make here is that the
   % relational data captures correctly the generative model, but if we
    %just join them and re-define units based in the joint data, then
    %there is intereference and contagion. Do you agree?}
For instance, the prestige of an author not only influences
  his or her acceptance rate, but it also has a {\em spill-over} effect on the acceptance rate of  his or her co-authors; this is called interference.
  Further, authors' qualifications can be {\em contagious}, meaning that if a junior author collaborates frequently with a
  senior author, then the overall quality of his or her own research may
  increase over time.
    \revm{To our knowledge, no tools exist that can model and address such intricate dependencies while allowing sound causal analysis accessible to a broad range of  data analysts.}
  \end{example}
  
  
  
  %\revm{Target audience of the relational causal learning }


  %\red{SR: WRITE A FEW LINES ABOUT OTHER DATASETS AND EXMAPLES.}
%   shows a simplified scheme of a
%   relational data we crawled from publicly available
%   websites~\cite{OpenReviwe,scopus}. The schema consists of the
%   entities $\mathit{People}$, $\mathit{Conference}$ and
%   $\mathit{Submission}$; and their relationships $\mathit{Author}$ and
%   $\mathit{Submitted}$; and a set of descriptive attributes such as
%   $\mathit{Decision}$ (whether a submission is accepted or rejected),
%   $\mathit{Blind}$ (whether a conference uses single or double-blind
%   reviewing) and $\mathit{Prestige}$ (whether an authors is afflicted
%   with a high-prestige institution). An interesting question that can
%   be investigated using \data\ is whether single-blind reviewing
%   confers any advantage to submissions from authors with high-prestige
%   institutions.  Specifically, we are interested in computing the
%   causal effect of authors' prestige on paper's decision. Note that
%   institutional prestige is perceived to be a significant predictor
%   for paper acceptance, thereby predictive analysis can be
%   perplexing. Additionally, this is challenging, as we are facing a
%   relational domain consisting of related heterogeneous
%   entities. Here, the institutional prestige belongs to the
%   $\mathit{Author}$ table, whereas the decision of a submission belong
%   to the $\mathit{Submission}$ table. Therefore, we don't have a unit
%   of study in in the sense of Rubin \cite{rubin1970thesis}. This rules
%   out using Rubin's causality out-of-the-box.  Furthermore, this
%   relational domain has a complex causal structure in which entities
%   exhibit {\em interference} and {\em contagion}. For instance,
%   prestige of an author not only influences their acceptance rate, but
%   also has a {\em spill-over} effect on the acceptance rate of their
%   co-authors, hence authors interfere. Moreover, authors
%   qualifications can be {\em contagious} over a course of
%   time. However, Pearl's causality does not permit us to describe such
%   complex relational causal dependencies between {\em multiple}
%   heterogeneous entities in a succinct way.
% 



\begin{figure}
    \centering
    \input{instance.tex}
    \caption{\revm{Fragment of the standard multi-relational database schema and a toy instance for \data.
    \cutr{obtained by
      integrating OpenReview, Scopus and Shanghai Rankings.
      }%\red{SR: CHANGE QUAL TO A SINGLE COLUMN} 
     % {\normalfont (The values shown are not real and not all attributes are shown.)}
     } }
     \vspace{-1cm}
    \label{fig:example_instance}
\end{figure}

\vspace{-2mm}
\textbf{Our contributions.~}  In this paper, we propose a declarative framework for {\em Causal
  Relational Learning} \cutr{a foundation for} 
 \revm{to support} causal inference over
\revm{relational data stored in multiple inter-related tables}. %domains. 
Our first contribution is a declarative language, \emph{\sys\ (Causal Relational Language)}, for representing causal background knowledge and assumptions \cutr{in relational domains} 
\revm{for relational data} ({\bf Section~\ref{sec:causal-framework}}). 
\sys\ can represent complex \revm{\emph{causal models}, i.e., potential causal dependence among the units}  using \cutr{just a few}
\revm{intuitive declarative} rules.  Given a database
instance\cut{(which we call a {\em skeleton})}, these rules are then
grounded to form a large ground causal graph, consisting of heterogeneous
units with complex inter-relationships.  \cut{To use the ground 
causal graphs for causal inference,
we make an important {\em structural homogeneity} assumption, which states that ground atoms of the same
type share the same {\em structural equations}; in other words, they share the same generative process.  Furthermore,} \revm{Most importantly,} details of the semantics of causal models are abstracted from the users, who \cutr{no longer}
\revm{do not} need to be statisticians;  instead, they can write {\em causal queries} in a high-level declarative language. \revm{We discuss the extensions in \sys\ over previous work in detail after we review the basic concepts and literature in causal analysis in Section~\ref{sec:background}.}
\par
Our second contribution
is a non-trivial extension of Pearl's $\Do$-operator to give semantics to complex causal queries about the \revm{average treatment effect}, and \emph{isolated}, \emph{relational}, and \emph{overall} effects of interventions ({\bf Section~\ref{sec:semantics}}).  When investigating the effect of authors' prestige on review scores (Example~\ref{ex:univdomain:causalmodel}), \revm{the isolated and relational effects respectively  measure to what extent the review scores are influenced by an author's own prestige
%. The relational effect measures to what extent the review scores of an author are influenced
and by the prestige of his or her collaborators}. We show that the overall effect is the sum of isolated and relational effects. 


% However, using \sys\ the users can pose these queries declaratively without
%without the need to know how these queries are mapped to the grounded causal model.
%The $do$-operator is defined as an
%intervention on one (or several) variables in a causal model.  In \sys,
%Our semantics defines how
%to map those treatments to $do$-operators on the grounded causal DAG.
\par
Our third contribution consists of an algorithm for answering 
causal queries from the given relational data ({\bf Section~\ref{sec:causal-queries:answering}}).  \revm{The algorithm detects a set of confounding covariates for a causal query given a causal graph and then makes relational causal analysis amenable to existing approaches by constructing a single unit table by embedding vectors of treatment, response, and covariates to smaller dimensions.}
\cutr{performs a static analysis of the causal query, and it constructs a unit-table specific to
the query and the relational causal model by identifying a set of attributes
that are sufficient for confounding adjustment.}   
\par
Finally, we present an end-to-end experimental evaluation of \sys\ ({\bf Section~\ref{sec:experiments}}) on %both
\revm{three real datasets -- \data\ \cite{OpenReview, scopus, shanghai} (an integrated review dataset as in Example~\ref{ex:univdomain:causalmodel},  \mimicdata\ \cite{mimic} (the Multiparameter Intelligent Monitoring in Intensive Care dataset, and \nisdata\ \cite{healthcare_cost_and_utilization_project_hcup_hcup_2006} (the Nationwide Inpatient Sample dataset)}), as well as on synthetic \data. 
%real and synthetic data 
We find that causal queries indeed provide quite different insights over real data compared to simple
associational queries that compute correlations, or compared to a naive causal analysis that
assumes homogeneous units and ignores relationships.  Over synthetic data (for which the ground truth is known),  \sys\ was
able to recover the ground truth. \revm{Over the real datasets, \sys\ found interesting answers for the following causal queries: (1) What is the effect of institutional prestige on reviewers' recommendations under single-blind and double-blind review processes? (2) What is the effect of not having insurance on patient mortality and length of stay? (3) What the effect of hospital size on affordability of healthcare?}


\cutr{\data, we present interesting findings on the causal effect of prestige on submission scores in single- versus double-blind venues. \red{SR: UPDATE AFTER OTHER EXPTS.}}

% In this paper, we propose a declarative framework for {\em Causal
%   Relational Learning}, a foundation for causal inference over
% relational domains. Specifically, we propose a declarative language, which allows us to define a {\em Relational Causal Model} for representing causal relationships between heterogeneous units, with
% complex relational structures, then allows us to formulate {\em Causal
%   Queries} over a given relational database, by using the same
% high-level declarative language.  We give semantics to the causal
% queries by proposing a new, non-trivial extension of Pearl's
% $\Do$-operator to relational causal models.  We then propose an
% algorithm for evaluating causal queries from the given data, by
% creating on-the-fly a table of units (specific to the query) and
% finding a sufficient set of {\em covariates} that should be adjusted
% for to remove confounding effects. 
% %%% We formalize complex causal queries about isolated and relational
% %%% effects in multi-relational settings. We propose techniques such
% %%% as {\em embedding relational data} for transforming relational
% %%% data into a flat table amenable for easy causal inference.
% Finally, we conduct an experimental evaluation of \sys\ on both real
% and synthetic data.  We make the following specific contributions.
 
 
%\dan{I think that this paragraph still needs work to explain our  contributions} \babak{revised} \dan{Sorry, it's still wasn't what it needs to be; here we need to brag about {\em our} system, and our system only.  I commented out the old paragraph in Latex, and replaced with this new one.  Please update: it is too long, and I probably did not capture well the contributions in Sections~\ref{sec:causal-query} and ~\ref{sec:causal-queries:answering}.  This paragraph needs to be written such that an expert reader can understand it, and appreciate it.}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%DAN'S
%Our first contribution is a declarative language, \emph{\sys\ (Causal Relational Language)}, for representing casual background knowledge and assumptions in relational domains.  The language can define complex causal models in relational domain using just a few rules.  Given a databaseinstance (which we call a {\em skeleton}), these rules are then
%grounded to form a large ground causal graph, consisting of heterogeneous
%units with complex inter-relationships.  In order to learn thestructural equations from the given data because, we make an important
%{\em homogeneity assumption}, by assumeing that all nodes of the same
%type have the same structural equations; in other words, nodes of the
%same type are governed by the same laws of physics.  Users do not need
%to be aware of the causal DAG, but instead write {\em causal queries}
%in the high-level declarative language.  Our second contribution
%consists of a non-trivial extension of Pearl's $Do$-operator to give
%semantics to these queries.  The $do$-operator is defined as an
%intervention on one (or several) variables in a causal DAG.  In \sys,
%however, the user asks causal queries in a declarative language, where
%the treatments are specified declaratively.  Our semantics defines how
%to map those treatments to $do$-operators on the grounded causal DAG.
%Our third contribution consists of an algorithm for answering the
%causal queries from the given data.  The algorithm performs a static%
%analysis on the causal query, and constructs a unit-table, specific to
%that query and the relational causal model, then finds the covariates,
%and computes the average treatment effect.  Finally, our fourth
%contribution consists of an experimental evaluation of \sys\ on both
%real data and synthetic data.  We find that causal queries provide
%indeed quite different insights over the real data than simple
%associational queries, or even than a naive causal analysis that
%assumes homogeneous units and ignores relationships.  We also found
%that, over synthetic data (where we had the ground truth) \sys\ was
%able to recover the ground truth with good accuracy.



%, then finds the covariates,
%and computes the average treatment effect.

%%% At the core of relational causal models is a declarative language that
%%% allows users to specify assumptions and background knowledge on the
%%% causal interactions among heterogeneous units, and to formulate causal
%%% queries. As oppose to predictive analysis, domain expert knowledge
%%% plays a critical role and is fundamentally required for causal
%%% inference \cite{pearl2009causal}. Pearl proposed causal graphs as a
%%% powerful mathematical tool for specifying these background
%%% knowledge. \footnote{The use of graphical models for capturing causal
%%%   relationships can be traced back to Sewall Wright's introduction of
%%%   path diagram in the early 1920~\cite{wright1921correlation}}
%%% However, as we argue in Section~\ref{sec:background} causal graphs are
%%% incapable of capturing causal relationships in complex relational
%%% domains in which heterogeneous units exhibit interference and
%%% contagion, e.g., the effect of collaborators of a professor on their
%%% student' learning. In contrast, in our declarative language called
%%% \sys\, users can specify complex background knowledge and their causal
%%% queries about relational domains with simple and intuitive
%%% Datalog-like rules.
%%% 

\cut{
In summary, we make the following contributions.  (1) We propose
Relational Causal Models with a declarative language
(Sec.~\ref{sec:causal-framework}).  (2) We introduce the semantics of
causal queries by extending the $do$-operator
(Sec~\ref{sec:causal-query}), (3) We develop a query answering
algorithm (Sec.~\ref{sec:causal-queries:answering}) and (4) we conduct
an experimental evaluation (Sec.~\ref{sec:experiments}).
}

%%% \dan{We should have one contribution per section.}  We make the
%%% following contributions: (1) We propose Relational Causal Molds, which
%%% lift Pearl's Causal Models to relational domains. (2) We propose \sys\
%%% a declarative language for capturing users’ assumptions and queries
%%% using simple Datalog-like rules. (2) We develop an underlying
%%% inference engine that automatically detects a sufficient set of {\em
%%%   covariates} that should be adjusted for to remove confounding
%%% effects. (3) We develop novel techniques such as {\em embedding} to
%%% transform relational data into a flat table amenable to easy causal
%%% inference.  (4) we answers a suite of causal queries considering
%%% relational and isolated effects. (5) We evaluate \sys\ on synthetic
%%% and real data, and illustrate the applicability of our method on
%%% estimating the causal effect of institutional prestige on the
%%% acceptance of papers under single-blind and double-blind review
%%% processes.
%%% 


%
%In this paper we develop the theory of {\em Relational Causal Models}, or ReCMs; grounded in Pearl's causal model  ReCMs provide a foundation for inferring causal inference from relational domain. ReCMs lift
%Pearl's causal models from representing causal relationship between attributes of homogeneous units, to heterogeneous units that are related with complex relational dependencies.  We extend Pearl's  $\Do$-operator to ReCMs, to capture complex interventions in relational domains.
\vspace{0.1cm}




%notion of causality studies in this paper is fundamentally different from prior works in query answer causality and responsibility and explanation \cite{RoyS14} and hypothetical reasoning  \cite{balmin2000hypothetical,lakshmanan2008if, deutch2013caravan} which aims to identify parts of the input that are correlated with query answers.  









%\sys\ extends the existing literature  (3) ground in the existing framework in causal inference, \sys\ articulate the assumptions required for making causal inference from relational data.



%to model a joint probability distribution over relational data amenable for probabilistic reasoning rather than causal inference ~\cite{Getoor:2007:ISR:1296231}.  However, using a causal interpretation of these dependency models in statistical relational learning, called {\em Relational Causal Graphical Models}, the authors in \cite{arbour2016inferring} studied interference in the context of social 

%{\em directed acyclic probabilistic entity-relationship} (DAPER)  \cite{heckerman2007probabilistic}.


% 
%\babak{add the work on homophily}

%Statistical Relational Learning (SRL) aims at unifying logic and probability to model a joint probability distribution over relational data amenable for probabilistic reasoning~\cite{Getoor:2007:ISR:1296231}. A plethora of models such as PRMs \cite{getoor2007probabilistic}, PSL, DAPER, PBNs, BLPs and MLNs has been proposed for SRL in the literature.  While our proposed framework for Causal Relational Learning, \sys, shares some similarities with some of these models, it is fundamentally motivated for causal reasoning. The closest SRL model to \sys\ are PRMs and  DAPER that extend the standard entity-relationship (ER) model to incorporates probabilistic dependencies. They can also be seen as a first-order extension of Bayesian Networks to relational data. However, there are two primary differences between \sys\ and these models. First, PRMs are dependency models that essentially define a joint probability distribution over all possible completions of a partially specified instance. In contrast \sys\ models the generative process of relational data. Here, the uncertainty is induced by hidden noise variables, {\em and prevails even
%when the entire relational data is available}. There has been prior attempt to 
%use use these models for causal inference from relational data, e.g., 


%At the core of ReCMs is a declarative language that can capture complex causal structure that are present in real-world scenarios and an inference ..





%that allows complex relational data to be mapped to the standard model used in statistics to perform causal inference. Using new techniques such as {\em embedding relational data}, RCMs can efficiently answer complex causal queries about the {\em interference} and {\em spill-over effect} of treatment strategies.




%in which the treatment is to instruct authors to manipulate their name/affliction in their submissions and the outcome is the submission's decision. 
%relational domain is challenging.  First, the domain consists of heterogeneous entity classes such as $\mathit{Author}$,  $\mathit{Submission}$ and  $\mathit{Conference}$ that are interconnected with relational dependencies (See Fig~\ref{fig:erdiagram}). Therefore, the units that receive a treatment can be different than the unit for which an outcome of interest in measured. In our case, the treatment of prestige applied to or withheld from each author, but response of decision measured for each submission. This rules out using Rubin's POF out-of-the-box. Furthermore, the treatment of  prestige of one author would affect the acceptance rate of all of his co-authors


%Presumably, authors from prestigious universities are submitting high-quality work, hence prestige is a {\em significant predictor} for acceptance, even when they are {\em causally independent}.


%This rules out using Rubin's POF out-of-the-box.

%Now, the 
 %Hence, even in double-blind reviewing we expect  author's prestige to be a significant predictor for paper acceptance.

%we expect a huge correlation between authors prestige 
%The entity-relationship diagram in Fig~\ref{fig:erdiagram} represents a simplified academic conference domain consist of three entity classes  $\mathit{Author}$,  $\mathit{Submission}$ and  $\mathit{Conference}$. Each author may have several submissions; and vice versa a submission may have several authors. A conference may receive several submissions, but each submission only associated to one conference. The attributes $\mathit{Impact}$, $\mathit{Productively}$ and $\mathit{Experience}$ describe the qualifications of the authors. $\mathit{Prestige}$ shows the prestige of the institution the authors are affiliated with. The attribute $\mathit{Quality}$ and $\mathit{Decision}$  respectively shows whether the submission has a decent quality and whether is it has been accepted or rejected for publication. 
%Finally, $\mathit{Blind}$ shows whether a conference follows a single vs double blind review policy.



%here is a many-to many relationship between  $\mathit{Author}$ and submissions and a one-to-many relationship between a $\mathit{Conference}$ and $\mathit{Submission}$.

%Consider the the causal graph in Fig~\ref{fig:dag:univer} representing a potential causal relationships in the paper authorship and scientific peer-review scenario. 

%The graph postulates the following causal relationship:
%\begin{itemize}
%    \item ``Prestige" of an author for a paper is dependent on the number of citations, experience and productivity of the author.
%    \item ``Quality" of the paper is also a function of citations of the authors and their experiences. The contribution of each author's covariates depends on their position in the list of authors for a given paper.
 %   \item ``Review-score" assigned by the group of reviewers to a paper submitted to a conference is dependent on the quality of the paper, rigor of the conference while it is hypothesized to depend on the prestige of the authors for single-blind venues. 
%\end{itemize}




%However, the causal DAG fails to capture confounding due to causal interaction of objects from related entities. For instance, to assess the effect of prestige of the author on review score of the submission one need to account for the authors' colleagues who the authors have worked with in the past as it might affect author's prestige.\harsh{here!} As shown in Fig~\ref{}(b), this example has: 1) \textit{interference}, because the tutoring received by one students affects the peer's outcomes; 2) \textit{contagion}, because related students are likely to study together and hence their outcomes affect each other's outcomes; and 3) \textit{induction}, because student tend to choose course which their friends choose and hence the treatment choice of one affects other's choice. Expressing causal interaction between the related objects in a network using non-structural equations (NSEs) is either impossible or tedious. 

%Our major contribution in this paper is the introduction {\em relational causal models}. We propose a richer language to describe {\em relational causal models} and an inference methodology which can capture complex causal dependencies that are present in real-world scenarios. The goal is to provide the theoretical foundation and tools for answering the following types of causal queries in relational settings:
%\begin{itemize}
   % \item What is the effect of tutoring sections on the grades of a student in a class?
  %  \item What is the effect of tutoring on the attendance rate of the student in that course?
   % \item what is the effect of one's lecture attendance in a class on one's grade in that class?
   % \item What is the effect of having team projects on the average grade in the class?
%\end{itemize}



==> response.tex <==
\section*{Response Letter for Paper 603:  ``Causal Relational Learning''}\label{sec:response}
We thank the reviewers for the revision opportunity and their clear and constructive reviews. We have made a major revision of the paper: we added experiments using two new real datasets from the medical domain, we rewrote the first three sections to make the paper accessible to a wider audience, and we made numerous other updates throughout the paper.  The paper is much improved now.  {\bf We have addressed all reviewers' comments as described in details below.}

Updates made in response to the comments are color-coded as follows. 
%In addition, we have improved the general presentation of the paper that we have not highlighted.
\begin{itemize}
	\itemsep0em
	\item \revm{Common changes for multiple reviewers and updates in the presentation of the paper are in RED}
	\item \reva{Reviewer 1 in BROWN.}
	\item \revb{Reviewer 2 in BLUE.}
	\item \revc{Reviewer 3 in MAGENTA.}
	\item \revd{Reviewer 4 in GREEN.}
\end{itemize}

%{The revised paper is appended after the response letter,  and the section/table/figure references can be clicked in the responses to reach the corresponding changes in the main paper.


\subsection{Meta-review}
\ques{Thank you for the submission. We would like to invite you to submit a revision; however, the required changes may require substantial effort. The reviewers will only reconsider the paper after the paper is improved and re-evaluate the paper for accept/reject after the revision. So we want to be clear that without substantial changes the revision will not be accepted and even with the changes, the reviewers will re-evaluate the paper to decide one way or another. I apologize for the bluntness here but I want to be clear so you can decide how to allocate your time and plan your strategy between doing this revision or waiting to submit to a different conference.} \revm{We are thankful to all the reviewers and the meta-reviewer for the revision opportunity. We have significantly updated the paper, as can be seen in the colored parts of the revised submission. The changes are also summarized below.\\}

\ques{In case you decide to resubmit, the following are major points that need to be addressed which came up during the discussion:}\\

\ques{- All reviewers find (parts of) the paper difficult to understand. The authors requested a 4th reviewer and a knowledgable 4th reviewer is sought but still has problems reading the paper with clarity. While we understand that this paper may require a certain expertise to evaluate, we will also appreciate it if it can be made more accessible to a knowledgable db reader.} \revm{We have made substantial updates of the presentation of the paper:
\begin{itemize}
    \item (Section~\ref{sec:intro}) We have updated the introduction  by simplifying the example, contributions, and motivations, and shortening its length. The related work is now moved to Section~\ref{sec:background}.
    \item (Section~\ref{sec:background})  We have updated  the background section   by simplifying the presentation, adding examples, and removing unnecessary details. 
    % \red{SR:  STILL HAVE THIS??} 
    We  also discussed some related work at the end of this section and add how our work  differs from existing  work. 
    \item (Section~\ref{sec:causal-framework}) Reviewer-4 had suggested merging Section  3 and 4, which  would have made it  a very long section. Instead, we now have  only the description of declarative framework of \sys\ and its declarative language in Section 3, and all the discussions on its semantics are  moved  to Section 4. We revised Section~\ref{sec:prelim} illustrating the conneection with the standard relational model and updating the examples. Now the running example in Figure~\ref{fig:example_instance} is in the standard relational form. Section~3.2 is updated too and contains the  syntax of causal rules specifying the background knowledge of users. As  the reviewers pointed  out, Section~3.3 earlier had the syntax and informal  semantics of causal rules, making the informal semantics difficult to follow, now it only has the syntax of the queries.
    Old Section 3.4 on ``Structural Homogeniety'' is  now  Section 4.1 (and is called ``Probability Distribution for \sys''),  as it is more related  to semantics of our model. Old Section 3.5 on discussions on heterogeneous data is now shortened and merged with new Section 4.1. This made Section 3 shorter and now it entirely focuses on the declarative framework of \sys. 
    
    
    \item (Section~\ref{sec:semantics}) Now the section starts with new Section 4.1 (moved from old Section 3.4) that  describes how `relational causal graphs' generalize Pearl's causal graphs, and how the probability distribution of the nodes in the relational causal graphs can be defined by aggregating their parents.   New Section 4.2 (old Section 4.1) that talks about treated and response units in heterogenous relational data is updated as well. New Section 4.3 describes the concept  of relational paths needed to define the semantics of queries in the next subsection (earlier part of old Section 4.4 that described the semantics of relational and isolated  queries). New Section 4.4 describes the semantics of all the query types described in new Section 3.3 (earlier distributed  in Section 4.2 and 4.5). The discussions in old Section 4.5 is now footnote 9, and the concept of aggregated  rules by aggregating attributes in old Section 4.3 is now moved to Section 3.2.4 as it is part of declarative framework in \sys.
    \item %Moved old section ???? to Section 3.2.4 as it is part of the specification language of \sys.
    (Section 5) Section 5.1 is simplified by removing some redundant details, the examples and Theorem 5.2 statements are revised. Similarly in Section 5.2, Table 1, examples, and discussions are updated. 
    \item (Section 6) Updates on the experiments are summarized below. As Reviewer-4 suggested, the embedding functions are moved out of the experiments section and is now Section 5.2.2. 
    \item The figures and tables have been moved and updated based on their new usage, and their captions are revised.
    \item The abstract and conclusions are updated too.
\end{itemize}
}

\vspace{5mm}

\ques{- The reviews also indicate concerns over the experimental evaluation. The experimental setting needs to be re-thought and evaluated to be more convincing.} \revm{We have restructured and extensively updated the experiments in Section~6. In addition to the old real and synthetic \data, it now includes experiments on two new real datasets: \mimicdata\ and \nisdata. 
%\sdata to scrutinize \sys's performance in depth. The section showcases \sys's ability to encode background knowledge, answer relational causal queries and recover ground-truth treatment effect.
The main updates in this section:
\begin{itemize}
    \item \mimicdata\: We thank Reviewer-4 for pointing us to the MIMIC dataset. \mimicdata\ \cite{mimic, mimiclink} is a freely available proprietary dataset that we obtained after completing required IRB protocols. The data is described in new Section 6.1 and has size 57GB after storing it in a Postgres database. We run queries against \mimicdata\ to test the causal effect of the lack of health insurance on patient mortality and length of stay.
    \item  \nisdata: We also did experiments on another healthcare dataset of 8 million hospital admissions across the US that we obtained from the Department of Health and Human Services, after completing a mandatory training course. After parsing and loading, the dataset consumes 15GB of disk space in Postgres. We query NIS to uncover the causal effect of hospital size on healthcare affordability.
    \item We have restructured Section~\ref{sec:experiments} by replacing some of the figures in previous version with articulate tables of results to accommodate new results from \mimicdata~ and \nisdata.
    \item We have also improved the presentation of the section in general.
\end{itemize}


}

\vspace{5mm}
\ques{In addition to these points, all points raised for attention in the detailed reviews must be addressed.} \revm{We have addressed all the comments and concerns raised by the reviewers as detailed below.}


\subsection{Reviewer 1}
\begin{itemize}
    \item(R1-W1) \ques{One of the main contributions of this work is "a non-trivial extension to Pearl's do-operator to give semantics to complex causal queries." The actual extension is not called out explicitly anywhere in Section 4, or at least explicit enough for a reader with limited familiarity of Pearl's do-operator to immediately appreciate.} \\
    %\harsh{NEED HELP.}
    \reva{We attempted to make the extensions clearer in the revision. Pearl's do-operator is reviewed in Section 2  along with standard causal DAGs and standard structural equations. Syntactically how \sys\ extends this framework is discussed in Section 3.2. Now the structural equations are associated with parameters for entities or relationships in relational data (compare equations in (9) with those in (2)), and the relational causal DAGs are extensions of causal DAGs as they contain grounding of variables to constants (compare Figure 3 with Figure 2). The semantics of this extension is discussed in new Section 4.1.}\\
    \item(R1-W2) \ques{Section 5.1 is extremely hard to follow, even with Example 5.3 and Observation 5.1. Particularly Equations 29 and 30 could benefit from some elaboration of the notation used.} \reva{We have revised this section by removing some redundant details and updating the examples and theorem statement.}\\ 
    %\harsh{NEED HELP.} \reva{REVISE 5.1}\\
    \item(R1-W3) \ques{For Section 5.2, the statement "Now all the causal queries in Section 4 can be estimated using standard statistical techniques for estimating (34) using the unit table D". Could you please elaborate on those, and whether other assumptions made elsewhere in the framework impact the validity of applying these techniques.}\\ \reva{The validity of the estimation process is contingent on the correctness of the relational causal model defined as a part of background knowledge. We have updated the Section~\ref{sec:cov-adjust} to explicitly mention the same.}\\
    
    \item(R1-D) \ques{I would like to thank the authors for their detailed response which addressed items I had listed below. However, I still have the same issues with the experiments that the other reviewers have raised. Thus, I feel this submission as it stands does not cross the bar for acceptance to SIGMOD until additional experiments are conducted and certain sections of the paper are modified to improve accessibility to a general audience.}\\
    \reva{We have updated experiments in Section~\ref{sec:experiments} to include more experiments from health and social science domains as requested by reviewers. We have also restructured the section to ensure to it flows intuitively for the reader. Please see our response to the metarevier's comment on experiments for a summary of changes.}\\
    \item(R1-R) \ques{The requested changes for the revision involve modifying several sections of the paper and strengthening the Experimental results with specifics listed by the reviewers for each.}\\ \reva{Please see our response to the metareviewer's comments. We have substantially updated the presentation of the paper as well as added new experiments on \mimicdata\ and \nisdata. }
\end{itemize}

\subsection{Reviewer 2}
\begin{itemize}
    \item (R2 - W2, D2) \ques{The Review Data, while an nice case study, is not nearly convincing. Most of the work on casual inference is in health/medical environment. While the authors mention such scenarios, none is considered. The review data is nice example, but not nearly convincing. It is unclear the motivation for the synthetic data since the data mirrors real life one. Perhaps, including other datasets, unrelated to review data, would help understand the values of this language.}\\
    \revb{See new Section~\ref{sec:experiments} and the response to metareviewer's comments. As suggested by the reviewers, it has been updated with new real data experiments from health/medical domain on \mimicdata~ and \nisdata. It has also been restructured to ensure reader find it easy to follow the results. Example of \data\ is still being used as a running example in the paper to illustrate all the concepts as \mimicdata\ and \nisdata\ has many attributes to use in an example. 
    %and hence \sdata\ is designed to mirror the \data.
    }
    
    \item (R2-W3 \ques{There is a great deal of effort put into the theoretical underpins of the proposed language, but there is little effort put into characterizing its properties: learning curve, efficiency, transparency, ease of communication.}\\
    
    \revb{We have updated the end of Section~\ref{sec:language:rules} (last paragraph and footnote) to discuss the properties of CaRL from the perspective of its intended users. We highlight CaRL's ease of use in comparison to existing techniques that rely on hand-tuning.}\\
    \item (R2 - D1,W1). \ques{It would be nice to have a discussion about the target audience of the proposed tool and whether it can be integrated with existing tools.}\\
    % \harsh{YET TO DO}\\
     \revb{In the conclusion (Section~\ref{sec:conclusion}), we have added a paragraph the target audience. In Section~\ref{sec:cov-adjust} We have added a paragraph which discusses  discusses how \sys~ is integrated with existing causal inference methods. }\\
    
    \item (R2 - D) \ques{I feel that a relevant, but missing, study is a comparison with a "baseline" of some sort. While reading the paper and trying to understand all the theoretical nuances, I could not by think of: How are things done nowadays?, How does CaRL help a bioinformatician or medical researcher?, What tools do those people use?, Would their tasks be improved with CaRL? But, I could not answer any of these questions while reading the paper.}\\
    \revb{As the existing frameworks do not support causal inference on relational datasets, the researchers currently cannot use them to perform causal inference when the data is in a relational setting. We believe, \sys~ will be able to bridge this gap and help bioinformatics, medical and social science researchers ask complex causal queries in a relational setup. Due to lack of literature on relational causal inference, we compare \sys's performance with causal inference performed on a universal table in Section~\ref{sec:experiments}. We treat this performance as a baseline performance as this might the most intuitive approach a research might traditionally use if they were to do causal inference on relational setup.}\\
\end{itemize}

\subsection{Reviewer 3}
\begin{itemize}
    \item (R3 - W1) \ques{The presentation needs significant improvement. The authors frequently abuse notations, which makes the paper hard to follow.}\\
    \revc{We appreciate the reviewer's suggestion on updating the presentation. We have reorganized the paper to ensure it is easy to follow for the readers. The updates are summarized in response to the meta-reviewer's comments and all updates have been color-coded for the reference of reviewers.}\\
    
    \item (R3 - W2, D5) \ques{Lack of theoretical analysis over the choice of embedding functions.}\\
    \revc{The intuitive idea behind embedding's efficacy is allowing the encoding the information of a variable sized vector into a fixed size vector. The embedding chosen aims at conserving underlying moments of the assumed distribution from the elements of variable sized vector is drawn. Thus, if the underlying assumed distribution resembles the true distribution then the summarization is lossless. However, we acknowledge that a thorough theoretical analysis on the choice of embeddings is out of scope of this paper. This paper primarily focuses on declarative framework, language, semantics, and query answering for \sys. The theoretical work on embeddings is an interesting future work as discussed in Section~\ref{sec:conclusion}.}\\
    
    \item (R3 - W3) \ques{The variety of the evaluated dataset and query is very limited.}\\
    \revc{See new Section~\ref{sec:experiments} and the response to metareviewer's comments. As suggested by the reviewers, it has been updated with new real data experiments from health/medical domain on \mimicdata~ and \nisdata. We have also added more examples of causal queries and their results. It has also been restructured to ensure the reader find it easy to follow the results. }\\
    
    \item (R3 - D1) \ques{This authors present a framework for conducting causal inference on complex relational database. This framework consists two parts:}
    \begin{itemize}
    \item A declarative language CaRL for expressing assumptions, causal queries;
    \item Inference engine that computes answers for the causal queries.\\
    \end{itemize}
    \revc{That is accurate.}\\
    
\item (R3 - D2)  \ques{The proposed framework supports the Average Treatment Effect (ATE) query and two additional types queries.}\\
\revc{That is accurate. Along with average treatment effect we can also estimate average overall effect, average individual effect and average relational effect.}\\

\item (R3 - D3)  \ques{Presentation/writing:
Overall, I found the presentation hard to follow. Many of the definitions/descriptions are quite confusing.}\\
 \revc{ We have reorganized the paper and revised it significantly so that it is easier to follow for the readers. Definitions and descriptions have also been reworded. Please see the  responses to metareviewer's comments for a summary of changes. The updates have been color coded for the reference of reviewers.}\\

\item (R3 - D4)  \ques{Declarative language CaRL:}
\begin{itemize}
    \item Given a database, do users need to define the relational causal model as well? If so, what is the syntax?
    \item For the causal rules, why specifying Q is necessary when the schema is already defined?\\
\end{itemize}
\revc{Section~\ref{sec:language} provides syntax for adding background knowledge to define relational causal model. The relational causal query is the question of interest while the relational causal rules only encode the background knowledge which allows \sys\ to figure out which variables to control for when answering the relational causal query.}
\\
\item (R3 - D5)  \ques{Methodology:}
\begin{itemize}
    \item Although studied through experiment, I'm not fully convinced why the embedding functions work. It is better to include some theoretical analysis.\\
\end{itemize}
\revc{Please see the combined answer in (R3 - W2, D5) above.}\\
\item (R3 - D6)  \ques{Experiments:}
\begin{itemize}
    \item The variety of the dataset/query is very limited.
    \item Extend the experiments to additional domain(s).\\
\end{itemize}
\revc{See Section~\ref{sec:experiments}. As suggested by the reviewer, it has been updated with new real data experiments from health/medical domain on \mimicdata~ and \nisdata. We have also added more examples of causal queries and their results. It has also been restructured to ensure reader find it easy to follow the results.}\\
\end{itemize}

\subsection{Reviewer 4}
\begin{itemize}
    \item (R4 - W1)  The paper can be structured better. E.g section 3 and 4 should be merged such that formal and informal definitions help each other.
    \revd{We considered merging old Sections 3 and 4, but it was resulting into a very long section. Therefore, we significantly restructured Sections 3 and 4 so that Section 3 entirely focuses on syntax of the \sys\ framework (and Section 3.3 no longer includes the informal descriptions of causal queries) whereas Section 4 entirely focuses on the semantics. Please see the responses to the metareviewer's comments for a summary of changes.\\}
    
    
    
    
    The explanation of different embedding should be also out of the experiment section and into the explanation parts.
    %\moe{Not sure what to say about the suggestion of merging sections 3 and 4}
    \revd{We have moved the explanation of embedding strategies from Section 6 to  Section~\ref{sec:embeddings}}.\\

    \item (R4 - W2) Poor experiment section. a) Only three queries are evaluated, one for each case. There authors should improve the number of queries used as well as a variety in complexity of the different queries used. b) different experiments use constraint and non-constrained settings without a valid explanation on why is one used over the other. c) There is no good comparison with other state of the art relational causal inference methods that are cited in the related work. for instance what datasets do they use? how does this method compare to others in their datasets? how do the other methods function on your new dataset?
    
    \revd{Please see the new Section 6 and response to metareviewer's comments on experinents. In particular,
    \begin{itemize}
        \item (a) we have extended the experiments to cover two additional datasets and new queries in the medical domain, MIMIC and NIS.
        \item (b) We are not exactly sure that we follow this comment. If the reviewer meant mentioning ATE vs. CATE (conditional average treatment effect) in the old experimental section, then please note that we have removed mention of CATE for simplicity in presentation (although those queries can be supported by \sys), and revised the presentation.  
        %\moe{I'm not sure I understand what the question is}
        \item (c) To the best of our knowledge, no other methods in causal inference can support relational data. In Section~\ref{sec:experiments} we compare CaRL to propensity score matching, a standard causal analysis method, on the universal table formed by joining all the tables in the relational data (Table 5).
    \end{itemize}}
\vspace{5mm}
    \item (R4 - W3) Adaptability to different domains. the papers starts with a motivation on the social sciences, but the method, dataset, examples and tests are all based on publication review process. The authors lack of explanation on how is this would apply in other domains or experiments such as using a different domain dataset. For instance the medical domain using MIMIC dataset of ICU patients would be an interesting relational dataset that is large and would really showcase the ideas exposes.
    
    \revd{We thank the reviewer for the suggestion to use MIMIC data. Now we have incorporated MIMIC into our experiments in Section~\ref{sec:experiments}. Additionally, we have also tested on the NIS---another large, relational healthcare dataset. Please see updated Section 6 and responses to metareviewer's comments.}
    
    \item (R4 - D1) Figure 1 is unnecessary.\\
    \revd{Figure 1 is removed. Please see updated Section~\ref{sec:intro}.}\\
    
    \item (R4 - D2) Example 1, Delete Significantly.\\
    \revd{We have shortened Example 1 significantly. Please see updated Section~\ref{sec:intro}.}\\
    
    \item (R4 - D3) Related work and Background analysis are not clear enough about what is the difference between other causal models from relational data and this work other than previous works being based on Statistical Relational Learning. 
    
    \revd{We have updated the Related Work paragraph in Section~\ref{sec:background} to be explicit about the differences between CaRL and works based on Statistical Relational Learning.}\\

    \item (R4 - D4) Range(A) in 3.1 ? 
    \revd{Range(A) was not used elsewhere, so we removed it.}\\
    
    \item (R4 - D5) Are attributes and Attribute functions the same? after some paragraphs A's are referred to as Attributes only.
    \revd{They are indeed the same. This has been made explicit in Section~\ref{sec:prelim}.}\\

    \item (R4 - D6) ATE is defined in section 2. and then again mentioned in section 3.3 without being explicit about the difference from related work and this work.\revd{One of the standard goals in causal inference is to compute ATE or average treatment effect, which is defined as the average difference of the effect of the response variables if the units receive treatment and do not receive treatment. Therefore, ATE is reviewed in Section 2. Computation of ATE is also supported by \sys\ as one of the causal queries. However, the standard approaches to compute ATE fail if we consider relational data as fundamental assumptions no longer hold. New Section 3.3 discusses how a user can specify an ATE query using \sys, new Section 4.4 discusses its semantics, and Section 5 discusses how we can answer such queries in relational data.}\\

    %\moe{I don't understand this question}

    \item (R4 - D7) In Page 6 the paragraph that explains relational queries is difficult to read. I don't understand the part "computes both isolated and relational effects of Prestige on reviewer scores if all coauthors from prestigious institutions." Is not clear the difference between relational and isolated. Is the condition the difference? how so? query (15) computes both? This question is resolved in section (4) with further explanation. This is why the structure should be adjusted.
    
    \revd{We have revised this paragraph to clarify the syntax, and referred to  the section 4.4.3 when the semantics of these queries are discussed in detail.}\\

    \item (R4 - D8) 4.2 how does this work when the intervention variable is not binary? for example prestige is a [0,1]?
    
    \revd{Following the standard assumption of binary treatments in the causality literature, we require the treatment attribute to be of binary domain, which can be enforced by using a threshold or a predicate on a non-binary domain.  In our example, prestige is 1 if the author is from a prestigious institution and 0 otherwise. How ``prestigious'' is defined may be dependent on many factors specific to the application (e.g., authors from top-k institutions by some ranking and for some value of k can have prestige = 1).}\\
    
    \item (R4 - D9) Definition 4.1 has redundancy.
    
    \revd{Redundancy has been removed from the definition, which is now Definition 4.2.}\\

    \item (R4 - D10) (30) is an equation not a theorem and Theorem 5.2 is not proved
    
    \revd{We now refer to (29) [previously (30)] as an equation. We defer the proof to the full version of the paper. There is an easy application of the proof (earlier Observation 5.1) that asks to condition on the parents of a node,  and we added some intuition why this works after the theorem. The proof of Theorem 5.2 is appended to the end of the response letter.}\\
    
    %\moe{Need to append proof to end}

    \item (R4 - D11) The Embedding concept and methods are fuzzy before reading the experimental section (6). It's mentioned in section (3) that it will be further explained in section 6 (experiments?) it should be discussed before experiment.
    
    \revd{We've moved the embedding methods to before the experiments section. They are now in section Section~\ref{sec:embeddings}.}\\

    \item (R4 - D12) In the paragraph "By mistakenly interpreting the naive correlation as causation, one might arrive at the conclusion that double blinding is not effective in reducing bias " where is this stated or proved by actually applying correlation instead of causation?
    \revd{We have replaced that sentence with concrete examples from the datasets of false discoveries. For example, in Section~\ref{sec:exp_end_to_end} Figure 6 (a) shows that correlation provides the false insight that double blinding is not effective in the \data\ dataset. Additionally, in the same section and using NIS dataset, we present a false discovery of 33\% decrease in affordability due to hospital size. We also show that our approach avoids this false discovery.}\\

    \item (R4 - D13) section 6. Q1: Is there a theorem 4.3? you mean proposition 4.3?
    
    \revd{It is indeed a proposition (now 4.4). This has been fixed.}\\

    \item (R4 - D14) why is experiment Q1(b) on synthetic and not real data?
    
    \revd{To evaluate the importance of encoding relations rather than ignoring them, we need the ground truth so a quantitative comparison of estimates can be made. We do not have this ground truth for real datasets as any unit can receive only one  of treatment and control.}\\

    \item (R4 - D15) why figure 7 is on CATE and the explanation is on ATE?
    
    \revd{We realized that the introduction of CATE in the experiments has caused confusion and so removed conditional effects from the paper. We now only report ATE and other effects defined in  Section 3.3.}\\
    
    \item Suggested a revision, I would like to see a strengthened experiment (see W2) and better write-up (see W1 and D1-8).
    
    \revd{Thank you for the revision opportunity. We have expanded the experiments and restructured the writing in earlier sections for increased clarity. Please see our responses to  the metareviewer's comments and the color-coded changes in the paper.}
\end{itemize}

